Unsupervised Quality Estimation for Neural Machine Translation

Quality Estimation (QE) is an important component in making Machine Translation (MT) useful in real-world applications, as it is aimed to inform the user on the quality of the MT output at test time. Existing approaches require large amounts of expert annotated data, computation and time for training. As an alternative, we devise an unsupervised approach to QE where no training or access to additional resources besides the MT system itself is required. Different from most of the current work that treats the MT system as a black box, we explore useful information that can be extracted from the MT system as a by-product of translation. By employing methods for uncertainty quantification, we achieve very good correlation with human judgments of quality, rivalling state-of-the-art supervised QE models. To evaluate our approach we collect the first dataset that enables work on both black-box and glass-box approaches to QE.

==> attention_head_layers.tex <==
To test whether a particular combination of attention heads and decoder layers may be more predictive of translation quality, we compute Pearson and Spearman correlation for all possible combinations. 
Tables \ref{tab:AW-Ent-PCC-eten} and \ref{tab:AW-Ent-SCC-eten} show the Pearson and Spearman correlation coefficients between entropy scores of attention weights and DA scores for Et-En language pair. We have computed entropy scores with ``end of sentence'' (EOS) mark and without it, because it is not a real token. In case of excluding the mark, we have renormalized the remaining attention weights.

\input{tables/attention_tables_eten_10K.tex}

As can be seen from the Tables \ref{tab:AW-Ent-PCC-eten} and \ref{tab:AW-Ent-SCC-eten}, the obtained Pearson and Spearman correlation coefficients are very diverse, for example,  the highest value of Pearson correlation coefficient for Estonian-English is almost 2.5 times higher than the smallest one (0.337 and 0.127, respectively). In most cases, the correlation coefficient is higher when we compute correlation coefficients without ``EOS'' mark. It is interesting to note that the average results over heads are diverse and the best average results are obtained for middle layers whereas average results over layers are not as varied. Although the average results over heads or over layers are still lower than the result obtained for the best head-layer combination.

\lisa{Analyze patterns between languages when all results will be available.}




==> discussion.tex <==
% \section{Model Confidence across NMT Systems}
\section{Discussion}\label{sec:discussion}

This Section provides a discussion of various questions related with experimental results presented above.

\subsection{Domain Shift}
%Above we have shown that expectation over probability distribution generated using MC dropout consistently methods based on non-calibrated output probability distribution, as well as a strong SOTA supervised QE system. 
Here we assess whether the improvement in correlation with MC dropout is achieved due to a better quantification of uncertainty.
%\todo{LS: is this what we are doing here? I thought we were checking whether sueprvised QE does worse because of domain shift}
One way to evaluate how well a model represents uncertainty is to measure the difference in model confidence under domain shift \cite{hendrycks2016baseline,lakshminarayanan2017simple,ovadia2019can}. A well calibrated model should produce low confidence estimates when tested on data points that are far away from the training data. %\todo{LS: This is confusing: a well calibrated model should produce that? or should it be robust to that? does that mean that the assumption is that we will always get low quality for out-of-domain?}. \mf{I think it does, the idea is that the model cannot be "certain" on OOD data even if the prediction turns out to be correct.} % As illustrated in \citet{gal2016dropout}, interpreting softmax probabilities as confidence can be misleading precisely because passing a point estimate of a function through softmax results in high confidence for points far away from the training data.

Overconfident predictions on out-of-domain sentences would undermine the benefits of unsupervised QE for NMT. This is particularly relevant given the current wide use of NMT for translating mixed domain data online. Therefore, we conduct a small experiment to compare model confidence on in-domain and out-of-domain data. We focus on Estonian-English language pair. We use the test partition of the MT training dataset as our in-domain sample. To generate the out-of-domain sample, we sort Wikipedia data (Section \ref{subsec:data}) by distance to the training data and select the top 500 segments with the largest distance score. To compute distance scores, we follow the strategy proposed by \citet{niehues2019modeling} that measures the distance between test and training data based on the hidden states of NMT encoder. 
%\paco{can we also add the pearson for these subsets?, If we have significant differences, then your point is stronger}\mf{I agree, but unfortunately we do not have the DA for the data that we use here.}

We measure model posterior probabilities for the translations of the in-domain and out-of-domain sample either obtained through standard decoding, or using MC dropout. Table \ref{tab:domain_shift} shows the results. The difference between MC-dropout average probabilities for in-domain vs. out-of-domain samples was found to be statistically significant under Student's T-test, with p-value $< 0.01$. Thus, expectation over predictive probabilities with MC dropout indeed provides a better estimation of model uncertainty for NMT, and thus can improve the robustness of unsupervised QE on out-of-domain data.

% There are many different ways to measure similarity or distance between sentences. 
% To find out-of-distribution examples it is necessary to look at the internal representations used by the MT model. 

% First, we run the encoder of the MT model on the source side of 1M segments randomly sampled from the training dataset and store the encoder hidden representation for every sentence. The encoder hidden states produced for each token are average to obtain the sentence-level representation. We then compute the same hidden representations for each source sentence in the Wikipedia testset. Next, we use k-nearest neighbor search to find the most similar training sentences for each test sentence. We use faiss library for implementation \cite{JDH17}. Finally, the test-train distance is computed as the distance to the overall most similar training sentence. 

\begin{table}[h]
\begin{center}
\begin{tabular}{|l | c c |} 
\hline
& IND & OOD \\ 
\hline
TP & -0.4397 & -0.4446 \\
D-TP & -0.5922 & -0.6849 \\
\hline
\end{tabular}
\end{center}
\caption{Average segment-level probabilities obtained through standard decoding (TP) or using MC dropout (D-TP) for in-domain (IND) and out-of-domain (OOD) samples.}
\label{tab:domain_shift}
\end{table}

% D-TP stdev for out-domain: 0.26266426877094434
% D-TP stdev for in-domain: 0.20963651718668688

% \input{attention_head_layers.tex}

\subsection{Model Confidence across NMT Systems}
\label{subsec:results_uncertainty_models}
%\paco{This section needs a better motivation. I would suggest something along the lines: We've shown that using the model confidence produces good correlations for many language pairs. One natural question is: how well do these findings generalize to other architectures and model parameters? Here we explore that question...}\mf{Added below.}
Results in previous Section suggest that using model probabilities results in fairly high correlation with human judgments for various language pairs. In this Section we study how well these findings generalize to different NMT systems. The list of model variants that we explore is by no means exhaustive and was motivated by common practices in MT and by the factors that can negatively affect model calibration (number of training epochs) or help represent uncertainty (model ensembling). Note that for this small-scale experiment we focus on the sequence-level translation probability (TP, as defined in Section \ref{subsec:probability}). 
%  Model calibration may depend on the specifics of the model architecture, training hyper-parameters or decoding strategy. For example, \citet{guo2017calibration} identify model capacity and weight decay as possible causes of miscalibration they observed. In this section we study how model architecture and training regime affect the relation between NMT output probabilities and perceived MT quality. 

%Besides the standard Transformer system, 
All system variants are trained using Fairseq implementation \cite{ott2019fairseq} for 30 epochs, with the best checkpoint chosen according the validation loss. Unless explicitly indicated otherwise, all variants are based on Transformer model from \citet{vaswani2017attention}.%\todo{LS: this is not clear, since we don't write below the ones that are not transformer. Maybe just remove this sentence and start each system description with Transformer or RNN.}\mf{But all of them except the RNN are in fact based on Transformer as underlying network architecture.} 

\subsubsection{Architectures and Training}

%We consider the following variants of NMT system architecture for our experiments:\footnote{
%}

\paragraph{Transformer} As a baseline for comparison, we use standard Transformer architecture from \citet{vaswani2017attention} with beam search decoding. %, an encoder-decoder model that relies on stacked self-attention and fully connected layers for both encoder and decoder.

\paragraph{Recurrent Neural Network} We look at state-of-the-art approach to NMT that preceded Transformer models: a standard attention-based RNN with LSTM cell as described by \citet{luong2015effective}.

\paragraph{Mixture of Experts} \citet{shen2019mixture} applied the mixture of experts (MoE) framework to capture the inherent uncertainty of the MT task and generate genuinely diverse hypotheses. A mixture model introduces a multinomial latent variable $z \in {1,...,K}$. The marginal likelihood is then decomposed as:
\begin{equation}
\begin{align}
p(y|x;\theta) &=& \sum_{z=1}^{K}p(y,z|x;\theta) \\
&=& \sum_{z=1}^{K}p(z|x;\theta)p(y|z,x;\theta)
\end{align}
\end{equation}
where $x$ and $y$ are the source and target sentences, respectively. The model is trained with EM algorithm where the E-step estimates the responsibilities of each expert and M-step update parameters $\theta$ with gradients weighted by their responsibilities. We use hard mixture model with uniform prior and $K=5$ mixture components. To produce the translations we generate from a randomly chosen component with standard beam search.

\paragraph{Ensembling} Previous work has used model ensembling as a strategy for representing model uncertainty \cite{lakshminarayanan2017simple,pearce2018uncertainty}. Here we take  a simple strategy for producing model ensemble typically used in NMT to improve translation quality. We train four Transformer models initialized with different random seeds. At decoding time predictive distributions from different models are combined by averaging. Note that MC dropout method discussed above can be interpreted as an ensemble model combination where the predictions are averaged over an ensemble of neural networks \cite{lakshminarayanan2017simple}.

\paragraph{Multilingual MT} multilingual approaches to MT have emerged relatively recently \citep{zeroshotMT,multilingscale}. Our expectation is that same approaches (like Transformer) when trained in a multilingual setting can yield translation outputs with completely different characteristics, thus enriching the diversity of text characteristics and types of translation errors in our experiments.

We follow the approach of multilingual multi-domain NMT \cite{multidomnmt,wmtmultinmt} where the system is additionally parametrized with the output language and text domain that are to be produced from the input segment. Each source-side token is accompanied by two factors (one for the output language and one for text domain), with their embeddings concatenated with the token embedding and the rest of the encoder being the same as a regular transformer.

\todo{four languages (en-et-ru-lv), domains, training corpora and fine-tuning on news}

% Note that both model ensembling represents model uncertainty, but by difference to MC dropout they require changes in system architecture and training algorithms. Conversely, MC dropout can be interpreted as an ensemble model combination where the predictions are averaged over an ensemble of neural networks \cite{lakshminarayanan2017simple}.

\subsubsection{Search}
Hypotheses spaces in NMT are very large and it is not feasible to explore them exhaustively. 

\paragraph{Beam search} This is traditionally used for decoding in NMT by exploring the search space in a greedy left-to-right manner retaining the top-N candidates with the highest probability. While effective to select a likely translation, beam search tends to over-represent frequent words while under-representing more rare words \cite{ott2018analyzing}, which may result in poorly calibrated model probabilities tending toward overconfidence. 
%We compare the following strategies for searching hypotheses space to standard decoding with beam search: 

\paragraph{Sampling} We generate translations one token at a time by sampling from the model conditional distribution $p(y_j|\vec{y}_{<j},\vec{x},\theta)$, until the end of sequence symbol is generated.

% Hypotheses spaces in NMT are very large and it is not feasible to explore them exhaustively. Beam search is an algorithm traditionally used for decoding in NMT. It explores the search space in a greedy left-to-right manner retaining the top-N candidates with the highest probability. As opposed to greedy search where the most probable word is selected at each time step, beam search explores multiple paths. It has been shown to provide a highly effective search strategy that helps to select the most likely translation under the model. However, as shown in \citet{ott2018analyzing}, beam search tends to over-represent frequent words while under-representing more rare words. This may result in poorly calibrated model probabilities tending toward overconfidence. To see whether this could be the case, we contrast beam search with simple sampling from the model distribution. In this latter case we generate translations one token at a time by sampling from the model conditional distribution $p(y_j|\vec{y}_{<j},\vec{x},\theta)$, until the end of sequence symbol is generated.

\paragraph{Diverse Beam Search} The resulting list of N-best translations in beam search lacks diversity, containing nearly identical target sequences. \citet{vijayakumar2016diverse} propose Diverse Beam Search, which promotes diversity by optimizing a diversity-augmented objective. It generates a list of diverse translation outputs and at the same time produces better top-1 candidates. %We analyse whether translation probabilities for the top-1 hypothesis obtained with Diverse Beam Search result in a better correlation with human judgments.

% Myle et al. (2018) show that sampling from the model better matches reference distribution while beam search overestimates frequent words. They also show that overall quality of samples is poorer than the results of beam search. They conjecture that this is due to the model spreading too much probability mass over the hypothesis space, thus underestimating the probability of individual hypotheses

% At decoding time combines prediction distributions from different models by averaging
% Models are the same model initialized with different random seed when training

\subsubsection{Results}

Table \ref{tab:uncertainty_across_models} shows Pearson correlation between sequence-level probabilities (TP) and DA judgments for translations generated by different NMT models for 400 segments (see Section \ref{subsec:data} for details on the data collection). First we show the correlation and DA for the standard Transformer model with beam search. Next, we present the results for different search algorithms. Finally, we show correlation and DA for the various network architectures (Recurrent Neural Network) or training procedures (ensembling, MoE and multilingual) described above. MoE corresponds to the probabilities produced by one mixture component, whereas MoE-all was produced by averaging probabilities from all mixture components. The last column shows the corresponding average DA judgments. 

% \todo{is the Ensemble not transformer? same for MoE? we need to state this in the systems descriptions}

% Table \ref{tab:da_across_models} shows the corresponding average DA judgments. DA-abs corresponds to absolute DA judgments produced on the scale 1-100 and DA-z corresponds to the same scores standardized for each annotator using their mean and standard deviation (see Section \ref{subsec:data} for details on how DA judgments were produced).

\input{tables/nmt_models_with_da.tex}

%Table \ref{tab:uncertainty_across_models} shows the results.
Interestingly, correlation between output probabilities and DA is not necessarily related to the quality of MT outputs. For example, sampling produces much higher correlation although the quality is much lower. This is in line with previous work that indicates that sampling results in better calibrated probability distribution \cite{ott2018analyzing}. System variants that promote diversity in NMT outputs (Diverse Beam Search and MoE) do not achieve any improvement in correlation over standard Transformer model, whereas ensemble model achieves the best results both in terms of MT quality and in terms of QE. We also note that applying temperature scaling improves the correlation without any drop in quality.

In addition, we study how the correlation with translation quality is affected by the number of training epochs. Longer training that leads to an increase in the accuracy of model predictions does not necessarily imply an increase in the calibration of its predictive probabilities or may even damage it \cite{guo2017calibration}.%\todo{LS: this is another good candidate to go}

It is not feasible to collect human judgments for translations produced by the system at each training epoch. Therefore, we generate translations for the test partition of the training set of the Estonian-English system and compute segment-level Meteor scores for the translations generated by our base Transformer system for $[1..60]$ training epochs. We compute the average Meteor scores and the correlation between segment-level Meteor scores and segment-level translation probabilities. Figure \ref{fig:calibration_by_epoch} shows the results. 

\begin{figure}[hbt!]
\centering
\includegraphics[width=0.5\textwidth]{figures/calibration_by_epoch.png}
\caption{Pearson correlation between translation quality and model probabilities, and translation quality over training epochs. Translation quality is measured using Meteor evaluation metric.}
\label{fig:calibration_by_epoch}
\end{figure}

Recall from Section \ref{subsec:data} that our training set for Estonian-English is relatively small with only 900K sentence pairs. Training a system for many epochs can induce overfitting. Interestingly, as the training continues test quality stabilizes whereas the relation between model probabilities and translation quality is deteriorated. During training after the model is able to correctly classify most of the training examples, the loss can be further minimized by increasing the confidence of predictions \cite{guo2017calibration}.


==> discussion_short.tex <==
% \section{Model Confidence across NMT Systems}
\section{Discussion}\label{sec:discussion}

This Section provides a discussion of various questions related with experimental results presented above.

\subsection{Domain Shift}
Here we assess whether the improvement in correlation with MC dropout is achieved due to a better quantification of uncertainty. One way to evaluate how well a model represents uncertainty is to measure the difference in model confidence under domain shift \cite{hendrycks2016baseline,lakshminarayanan2017simple,ovadia2019can}. A well calibrated model should produce low confidence estimates when tested on data points that are far away from the training data. 

Overconfident predictions on out-of-domain sentences would undermine the benefits of unsupervised QE for NMT. This is particularly relevant given the current wide use of NMT for translating mixed domain data online. Therefore, we conduct a small experiment to compare model confidence on in-domain and out-of-domain data. We focus on Estonian-English language pair. We use the test partition of the MT training dataset as our in-domain sample. To generate the out-of-domain sample, we sort Wikipedia data (Section \ref{subsec:data}) by distance to the training data and select the top 500 segments with the largest distance score. To compute distance scores, we follow the strategy proposed by \citet{niehues2019modeling} that measures the distance between test and training data based on the hidden states of NMT encoder. 

We measure model posterior probabilities for the translations of the in-domain and out-of-domain sample either obtained through standard decoding, or using MC dropout. TP has the average values of -0.440 and -0.445 for in-domain and out-of-domain data respectively, whereas for D-TP these values are -0.592 and -0.685. The difference between in-domain and out-of-domain confidence estimates obtained by standard decoding is negligible. The difference between MC-dropout average probabilities for in-domain vs. out-of-domain samples was found to be statistically significant under Student's T-test, with p-value $< 0.01$. Thus, expectation over predictive probabilities with MC dropout indeed provides a better estimation of model uncertainty for NMT, and therefore can improve the robustness of unsupervised QE on out-of-domain data.

% D-TP stdev for out-domain: 0.26266426877094434
% D-TP stdev for in-domain: 0.20963651718668688

\subsection{Model Confidence across NMT Systems}
\label{subsec:results_uncertainty_models}
%\paco{This section needs a better motivation. I would suggest something along the lines: We've shown that using the model confidence produces good correlations for many language pairs. One natural question is: how well do these findings generalize to other architectures and model parameters? Here we explore that question...}\mf{Added below.}
Results in previous Section suggest that using model probabilities results in fairly high correlation with human judgments for various language pairs. In this Section we study how well these findings generalize to different NMT systems. The list of model variants that we explore is by no means exhaustive and was motivated by common practices in MT and by the factors that can negatively affect model calibration (number of training epochs) or help represent uncertainty (model ensembling). For this small-scale experiment we focus on Estonian-English. For each system variant we translated 400 sentences from the test partition of our dataset and collected the DA accordingly. 

%  Model calibration may depend on the specifics of the model architecture, training hyper-parameters or decoding strategy. For example, \citet{guo2017calibration} identify model capacity and weight decay as possible causes of miscalibration they observed. In this section we study how model architecture and training regime affect the relation between NMT output probabilities and perceived MT quality. 

% Besides the standard Transformer system, 
% All system variants are trained using Fairseq implementation \cite{ott2019fairseq} for 30 epochs, with the best checkpoint chosen according the validation loss. Unless explicitly indicated otherwise, all variants are based on Transformer model from \citet{vaswani2017attention}.%\todo{LS: this is not clear, since we don't write below the ones that are not transformer. Maybe just remove this sentence and start each system description with Transformer or RNN.}\mf{But all of them except the RNN are in fact based on Transformer as underlying network architecture.} 

\subsubsection{Architectures and Training}

\paragraph{Transformer} As a baseline for comparison, we use standard Transformer architecture from \citet{vaswani2017attention} with beam search decoding. %, an encoder-decoder model that relies on stacked self-attention and fully connected layers for both encoder and decoder.

\paragraph{Recurrent Neural Network} We look at state-of-the-art approach to NMT that preceded Transformer models: a standard attention-based RNN with LSTM cell as described by \citet{luong2015effective}.

\paragraph{Mixture of Experts} \citet{shen2019mixture} applied the mixture of experts (MoE) framework to capture the inherent uncertainty of the MT task where the same input sentence can have multiple correct translations. A mixture model introduces a multinomial latent variable to control generation and produce a diverse set of MT hypotheses. We use hard mixture model with uniform prior and $K=5$ mixture components. To produce the translations we generate from a randomly chosen component with standard beam search.

\paragraph{Ensembling} Previous work has used model ensembling as a strategy for representing model uncertainty \cite{lakshminarayanan2017simple,pearce2018uncertainty}. Here we take  a simple strategy for producing model ensemble typically used in NMT to improve translation quality. We train four Transformer models initialized with different random seeds. At decoding time predictive distributions from different models are combined by averaging. Note that MC dropout method discussed above can be interpreted as an ensemble model combination where the predictions are averaged over an ensemble of neural networks \cite{lakshminarayanan2017simple}.

\subsubsection{Search}
Hypotheses spaces in NMT are very large and it is not feasible to explore them exhaustively. 

\paragraph{Beam search} This is traditionally used for decoding in NMT by exploring the search space in a greedy left-to-right manner retaining the top-N candidates with the highest probability. While effective to select a likely translation, beam search tends to over-represent frequent words while under-representing more rare words \cite{ott2018analyzing}, which may result in poorly calibrated model probabilities tending toward overconfidence. 
%We compare the following strategies for searching hypotheses space to standard decoding with beam search: 

\paragraph{Sampling} We generate translations one token at a time by sampling from the model conditional distribution $p(y_j|\vec{y}_{<j},\vec{x},\theta)$, until the end of sequence symbol is generated.

\paragraph{Diverse Beam Search} The resulting list of N-best translations in beam search lacks diversity, containing nearly identical target sequences. \citet{vijayakumar2016diverse} propose Diverse Beam Search, which promotes diversity by optimizing a diversity-augmented objective.
\subsubsection{Results}

% Pearson correlation between sequence-level probabilities (TP) and DA judgments for translations generated by different NMT models for 400 segments (see Section \ref{subsec:data} for details on the data collection). First we show the correlation and DA for the standard Transformer model with beam search. Next, we present the results for different search algorithms. Finally, we show correlation and DA for the various network architectures (Recurrent Neural Network) or training procedures (ensembling, MoE and multilingual) described above. MoE corresponds to the probabilities produced by one mixture component, whereas MoE-all was produced by averaging probabilities from all mixture components. The last column shows the corresponding average DA judgments. 


\input{tables/nmt_models_with_da.tex}

Table \ref{tab:uncertainty_across_models} shows the results. Interestingly, correlation between output probabilities and DA is not necessarily related to the quality of MT outputs. For example, sampling produces much higher correlation although the quality is much lower. This is in line with previous work that indicates that sampling results in better calibrated probability distribution \cite{ott2018analyzing}. System variants that promote diversity in NMT outputs (Diverse Beam Search and MoE) do not achieve any improvement in correlation over standard Transformer model, whereas ensemble model achieves the best results both in terms of MT quality and in terms of QE. We also note that applying temperature scaling improves the correlation without any drop in quality.

\subsubsection{Training Epochs}

In addition, we study how the correlation with translation quality is affected by the number of training epochs. Longer training that leads to an increase in the accuracy of model predictions does not necessarily imply an increase in the calibration of its predictive probabilities or may even damage it \cite{guo2017calibration}.%\todo{LS: this is another good candidate to go}

It is not feasible to collect human judgments for translations produced by the system at each training epoch. Therefore, we generate translations for the test partition of the training set of the Estonian-English system and compute segment-level Meteor scores for the translations generated by our base Transformer system for $[1..60]$ training epochs. We compute the average Meteor scores and the correlation between segment-level Meteor scores and segment-level translation probabilities. Figure \ref{fig:calibration_by_epoch} shows the results. 

\begin{figure}[hbt!]
\centering
% \includegraphics[width=0.5\textwidth]{figures/calibration_by_epoch.png}
\includegraphics[scale=0.35]{figures/calibration_by_epoch.png}
\caption{Pearson correlation between translation quality and model probabilities, and translation quality over training epochs. Translation quality is measured using Meteor evaluation metric.}
\label{fig:calibration_by_epoch}
\end{figure}

Recall from Section \ref{subsec:data} that our training set for Estonian-English is relatively small with only 900K sentence pairs. Training a system for many epochs can induce overfitting. Interestingly, as the training continues test quality stabilizes whereas the relation between model probabilities and translation quality is deteriorated. During training after the model is able to correctly classify most of the training examples, the loss can be further minimized by increasing the confidence of predictions \cite{guo2017calibration}.


==> discussion_short_v2_no_domain_shift.tex <==
\section{Discussion}\label{sec:discussion}

Results in previous Section suggest that using model probabilities results in fairly high correlation with human judgments for various language pairs. In this Section we study how well these findings generalize to different NMT systems. The list of model variants that we explore is by no means exhaustive and was motivated by common practices in MT and by the factors that can negatively affect model calibration (number of training epochs) or help represent uncertainty (model ensembling). For this small-scale experiment we focus on Estonian-English. For each system variant we translated 400 sentences from the test partition of our dataset and collected the DA accordingly. As baseline, we use a standard Transformer model with beam search decoding. All system variants are trained using Fairseq implementation \cite{ott2019fairseq} for 30 epochs, with the best checkpoint chosen according the validation loss.\footnote{Unless explicitly indicated otherwise, all variants are based on Transformer model from \citet{vaswani2017attention}.}

\textbf{First}, we consider three system variants with differences in architecture or training:
\begin{itemize}
    \itemsep0em 
    \item RNN-based NMT \cite{bahdanau2014neural,luong2015effective}
    \item Mixture of Experts (MoE) \cite{shen2019mixture}
    \item Model ensemble \cite{garmash2016ensemble}
\end{itemize}

\citet{shen2019mixture} use the \emph{MoE} framework to capture the inherent uncertainty of the MT task where the same input sentence can have multiple correct translations. A mixture model introduces a multinomial latent variable to control generation and produce a diverse set of MT hypotheses. In our experiment we use hard mixture model with uniform prior and 5 mixture components. To produce the translations we generate from a randomly chosen component with standard beam search.

Previous work has used \emph{model ensembling} as a strategy for representing model uncertainty \cite{lakshminarayanan2017simple,pearce2018uncertainty}. In NMT ensembling has been used to improve translation quality. We train four Transformer models initialized with different random seeds. At decoding time predictive distributions from different models are combined by averaging.\footnote{Note that MC dropout method discussed in previous Section can be interpreted as an ensemble model combination where the predictions are averaged over an ensemble of NNs \cite{lakshminarayanan2017simple}.}

\textbf{Second}, we consider two alternatives to beam search: diverse beam search \cite{vijayakumar2016diverse} and sampling. For sampling, we generate translations one token at a time by sampling from the model conditional distribution $p(y_j|\vec{y}_{<j},\vec{x},\theta)$, until the end of sequence symbol is generated.

\textbf{Third}, we report the results for the temperature scaling method presented in \S \ref{subsec:uncertainty}. For comparison, we also compute the D-TP metric for the standard Transformer model on the subset of 400 segments considered for this experiment.

\input{tables/nmt_models_with_da.tex}

% Table \ref{tab:uncertainty_across_models} shows the results. Interestingly, correlation between output probabilities and DA is not necessarily related to the quality of MT outputs. For example, sampling produces much higher correlation although the quality is much lower. This is in line with previous work that indicates that sampling results in better calibrated probability distribution than beam search \cite{ott2018analyzing}. System variants that promote diversity in NMT outputs (diverse beam search and MoE) do not achieve any improvement in correlation over standard Transformer model, whereas ensemble model achieves the best results both in terms of MT quality and in terms of QE. We also note that applying temperature scaling improves the correlation without any drop in quality.

Table \ref{tab:uncertainty_across_models} shows the results. Interestingly, correlation between output probabilities and DA is not necessarily related to the quality of MT outputs. For example, sampling produces much higher correlation although the quality is much lower. This is in line with previous work that indicates that sampling results in better calibrated probability distribution than beam search \cite{ott2018analyzing}. System variants that promote diversity in NMT outputs (diverse beam search and MoE) do not achieve any improvement in correlation over standard Transformer model

The best results are achieved by both in terms of quality and QE are achieved by model ensembling, which provides additional evidence that better uncertainty quantification in NMT improved correlation with human judgments. MC dropout and temperature scaling achieve very similar results.\footnote{The practical implementation of temperature scaling, however, is limited by the need for tuning the value of the scaling constant.} We recommend using either of these three methods for building NMT system with unsupervised QE.

\subsection{NMT Calibration across Training Epochs}

The final question we address is how the correlation between translation probabilities and translation quality is affected by the amount of training. We train our base Estonian-English Transformer system for 60 epochs. We generate and evaluate translations after each epoch. We use the test partition of the MT training set and assess translation quality with Meteor evaluation metric. Figure \ref{fig:calibration_by_epoch} shows the average Meteor scores (blue) and Pearson correlation (orange) between segment-level Meteor scores and translation probabilities from the MT system for each epoch.

\begin{figure}[hbt!]
\centering
% \includegraphics[width=0.5\textwidth]{figures/calibration_by_epoch.png}
\includegraphics[scale=0.35]{figures/calibration_by_epoch.png}
\caption{Pearson correlation between translation quality and model probabilities (orange); and translation quality measured with Meteor (blue) over training epochs.}
\label{fig:calibration_by_epoch}
\end{figure}

Interestingly, as the training continues test quality stabilizes whereas the relation between model probabilities and translation quality is deteriorated. During training, after the model is able to correctly classify most of the training examples, the loss can be further minimized by increasing the confidence of predictions \cite{guo2017calibration}. Thus, while longer training does not affect output quality but damages calibration.

%% previous version:
% In addition, we study how the correlation with translation quality is affected by the number of training epochs. Longer training that leads to an increase in the accuracy of model predictions does not necessarily imply an increase in the calibration of its predictive probabilities or may even damage it \cite{guo2017calibration}.%\todo{LS: this is another good candidate to go}

% It is not feasible to collect human judgments for translations produced by the system at each training epoch. Therefore, we generate translations for the test partition of the training set of the Estonian-English system and compute segment-level Meteor scores for the translations generated by our base Transformer system for 60 training epochs. We compute the average Meteor scores and the correlation between segment-level Meteor scores and segment-level translation probabilities. Figure \ref{fig:calibration_by_epoch} shows the results. 

% Recall from Section \ref{subsec:data} that our training set for Estonian-English is relatively small with only 900K sentence pairs. Training a system for many epochs can induce overfitting. Interestingly, as the training continues test quality stabilizes whereas the relation between model probabilities and translation quality is deteriorated. During training after the model is able to correctly classify most of the training examples, the loss can be further minimized by increasing the confidence of predictions \cite{guo2017calibration}.


==> experiments.tex <==
\section{Experiments and Results}
\label{sec:experiments}
Below we analyse how our unsupervised QE indicators correlate with human judgments.

\subsection{Settings}

\paragraph{Data} We use the dataset and NMT models described in Section \ref{subsec:data}. To make the results comparable with the Predictor-Estimator approach described above, we use the test (1K) partition of the dataset for evaluation, whereas train (7K) and dev (1K) partitions are used to train the supervised QE system.

\paragraph{Benchmark systems}
We compare the performance of the proposed unsupervised QE measures against the best performing approach to supervised QE with available open-source implementation, namely the Predictor-Estimator architecture~\cite{kim2017predictor} provided by OpenKiwi toolkit ~\cite{openkiwi}. This model is an encoder-decoder RNN ({\it predictor}), which predicts words along with context representation from an attention mechanism. These representations are used as input for a unidirectional RNN ({\it estimator}) that produces quality estimates. We trained a Predictor model on the same data as the NMT systems, while the Estimator model was trained on the 7K DA judgement data. % (see Section~\ref{subsec:data}). %For each of the two models, we used the default training configuration provided by~\citet{openkiwi}.

As another point of comparison, we compute popular reference-based evaluation metrics: BLEU \cite{papineni2002bleu,Lin:2004orange}, Meteor \cite{denkowski2014meteor}, TER \cite{snover2006study} and ChrF \cite{popovic:2015:WMT2015}, for Estonian-English, for which we have independently collected reference translations. % (see Section \ref{subsec:data}).

\input{tables/summary_table_all_languages_pearson}

\subsection{Correlation with Human Judgments}

Table \ref{tab:uncertainty_indicators} shows Pearson correlation with human judgments for the different unsupervised QE indicators described in Section \ref{sec:unsupervised_quality_estimation}, as well as for the supervised QE system and the reference-based automatic evaluation metrics presented above. Unsupervised QE indicators are further grouped as follows: group I corresponds to the measurements obtained with standard decoding (Section \ref{subsec:probability}); group II contains indicators computed using MC dropout (Section \ref{subsec:uncertainty});\footnote{We use dropout rate of 0.3 and apply dropout before each weight layer. We perform $N=30$ inference passes to obtain posterior probability distribution for estimating model uncertainty. Below we test how using a smaller or a larger the number of inference passes affects QE results (see Figure \ref{fig:forward_passes}).} and
group III contains the results for attention-based indicators (Section \ref{subsec:attention}).
% Table \ref{tab:uncertainty_indicators} shows Pearson correlation with human judgments for the different unsupervised QE indicators described in Section \ref{sec:unsupervised_quality_estimation}. The first group of measurements were obtained through standard decoding (Section \ref{subsec:probability}). The second group of indicators were computed using MC dropout (Section \ref{subsec:uncertainty}). The third group contains the results for attention-based indicators (Section \ref{subsec:attention}). The middle group contains the results for supervised QE state-of-the-art approaches, while the last group shows standard reference-based metrics.
We use Hotelling-Williams test to compute significance of the difference between dependent correlations \cite{Williams:1959} with p-value $< 0.05$. Results that are not significantly outperformed by any method are underlined; results that are not significantly outperformed by any other method from the same group are marked in bold.
%\todo{I split supervised from reference-based, they are different. Can you please re-check the significance? is AW:best head/layer not better than all others in the same group (bold)?}

\begin{figure*}[ht]
\centering
\begin{subfigure}  
    \includegraphics[width=0.45\textwidth]{figures/token-probas_seg19.png}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.45\textwidth]{figures/token-probas_seg313.png}
\end{subfigure}
\caption{Two examples of Estonian-English translations with very similar overall sentence-level probability (-0.50 and -0.48 for the first and second sentence, respectively) but very different patterns in the sequence of token-level probabilities.}
\label{fig:token_probabilities}
\end{figure*}

\input{tables/example_variation_v2.tex}

We observe that the simplest measure that can be extracted from NMT, sequence-level probability (\emph{TP}), already performs competitively, in particular for the medium-resource language pairs. \emph{TP} is consistently outperformed by \emph{D-TP} indicating that NMT output probabilities are not perfectly calibrated. This outcome confirms our hypothesis that estimating model uncertainty improves correlation with perceived translation quality. Furthermore, our unsupervised approach outperforms current state-of-the-art in supervised QE. These results position the proposed unsupervised QE methods as an attractive alternative to the supervised approach, as they can be extracted as a by product of translation with no need to access any additional resources besides the NMT system itself. 

Another general observation is that for both unsupervised and supervised methods performance varies considerably across language pairs. %Our dataset covers very different scenarios in MT development and evaluation. As described in Section \ref{subsec:data}, we have a full spectre of language pairs according to the amount of data available for MT training.
The highest correlation is achieved for the medium-resource languages, whereas for high-resource language pairs it is drastically lower. The main reason for this difference is a lower variability in translation quality for high-resource language pairs. Figure \ref{fig:distribution_across_languages} shows the distribution of DA scores and the scatter plots for the Romanian-English, which has the best correlation results, and English-German with the lowest correlation for all quality indicators. Romanian-English contains a substantial number of high-quality sentences, but the rest of the translations are uniformly distributed across the quality range. The distribution for English-German is highly skewed, as the vast majority of the translations are of high quality. In this case capturing meaningful variation appears to be more challenging, as the differences reflected by the DA judgments may be more subtle than any of the QE methods is able to reveal. % \paco{It is interesting that here we're seeing the opposite effect as with the WMT datasets.}

The reason for a lower correlation for Sinhala and Nepalese is different. For unsupervised indicators it can be due to the difference in model capacity\footnote{Models for these languages were trained using Transformer-Big architecture from \citet{vaswani2017attention}.} 
%Transformer for the rest of the language pairs)\mf{Vishrav, could you please confirm this?}
and the amount of training data. On the one hand, as demonstrated by \citet{guo2017calibration}, increasing depth and width of the model may negatively affect calibration. On the one hand, due to the small amount of training data the model can overfit resulting in inferior results both in terms of translation quality and in terms of correlation. It is noteworthy, however, that supervised QE system suffers a larger drop in performance than unsupervised indicators, as the predictor component of this system requires large amounts of parallel data for successful training. We suggest, therefore, that unsupervised QE is more stable in low-resource scenarios than supervised approaches. 

% Figure X shows the We observe that the trends described above are maintained \textbf{across language pairs} \todo{LS: not all of them yet, let's wait and see}. Thus, D-TP consistently outperforms the indicators based on model probability distribution, as well as the strong state-of-the-art system for supervised QE. Correlation values, however, vary considerably across language pairs. To gain insight into this difference, we look at the scatter plots and the distribution of DA scores for Romanian-English and English-German. As shown in Figure \ref{fig:distribution_across_languages}, Romanian-English contains a substantial number of high-quality sentences, but the rest of the translations are uniformly distributed across the quality range. The distribution for English-German is highly skewed, as the vast majority of the translations are of high quality. In this case capturing meaningful variation appears to be more challenging, as the differences reflected by the DA judgments may be more subtle than any of the \paco{(unsupervised)} QE methods is able to reveal.  \paco{It is interesting that here we're seeing the opposite effect as with the WMT datasets.}

We now look in more detail at the three groups of unsupervised measurements in Table \ref{tab:uncertainty_indicators}.

\paragraph{Group I} For the first group, average entropy of the softmax output ($\mathrm{Soft\mbox{-}Ent}$) and dispersion of the values of token-level probabilities ($\mathrm{Sent\mbox{-}Var}$) produce competitive results, with a substantial improvement over sequence-level translation probability for some of the language pairs. (i) Softmax entropy captures uncertainty of the output probability distribution, which appears to be a more accurate reflection of the overall translation quality. (ii) The dispersion of the values of token-level probabilities captures a pattern in the sequence of token-level probabilities that helps detect low-quality translation. Consider the example in Figure \ref{fig:token_probabilities}. It shows two MT outputs. Both are translations from Estonian into English. They have the absolute DA scores of 62 and 1, respectively, the first sentence being clearly superior in quality. But the difference in their sentence-level log-probability is negligible: -0.50 and -0.48 for the first and second translations, respectively. By contrast, the sequence of token-level probabilities for these two sentences looks very differently, as the second sentence has larger variation in the log-probabilities for adjacent words, with very high probabilities for high-frequency function words and low probabilities for content words. %\todo{LS: this is another candidate to go if we need space as I'm not sure it adds much to the paper, even though it's super interesting. we may be able to explain without plots} %We suggest that further analysis of the patterns of token-level probabilities in translated sequences can lead to even better correlation results.

\paragraph{Group II} The best results are achieved by the $\mathrm{D\mbox{-}TP}$ metric that measures the expectation over posterior probabilities obtained using MC dropout. %This confirms our hypothesis that a better representation of model uncertainty leads to a higher correlation with human judgements of MT quality. 
Interestingly, D-Var has a much lower correlation, since by only capturing variance it ignores the actual probability estimate assigned by the model to the given output.\footnote{This is in contrast with the work by \citet{wang2019improving} where D-Var appears to be one of the best performing metric for NMT training with back-translation demonstrating an essential difference with the QE task.}

Table \ref{tab:linguistic_variation} provides an illustration of how model uncertainty captured by MC dropout reflects the quality of MT output. The first example contains a low quality translation, with a high variability in MT hypotheses obtained with MC dropout. By contrast, MC dropout hypotheses for the second high-quality example are very similar and in fact constitute valid linguistic paraphrases of each other. This fact is directly exploited by the $\mathrm{D\mbox{-}Lex\mbox{-}Sim}$ metric that measures the variability between MT hypotheses generated with perturbed model parameters and performs on pair with $\mathrm{D\mbox{-}TP}$. $\mathrm{D\mbox{-}Lex\mbox{-}Sim}$, besides capturing model uncertainty, reflects the potential complexity of the source segments, as the number of different possible translations of the sentences is an indicator of its inherent ambiguity. It should be noted, however, that this is a less practical method, since generating additional translations is more costly than re-scoring an already generated MT output multiple times.

A question that arises for the practical application of $\mathrm{D\mbox{-}TP}$ is how the results would be affected by the number of stochastic forward passes. Figure \ref{fig:forward_passes} shows Pearson correlation with human judgments for our $\mathrm{D\mbox{-}TP}$ metric as a function of the number of stochastic forward passes of MC dropout for Romanian-English and Estonian-English, where this metric brings the largest gains over sequence-level probability. Based on the results in Figure \ref{fig:forward_passes}, we suggest using $N=20$ as increasing N beyond 20 does not give any improvement in correlation.

\begin{figure}[ht]
\centering
    \includegraphics[width=0.45\textwidth]{figures/n_forward_passes.png}
\caption{Pearson correlation with human judgments for our $\mathrm{D\mbox{-}TP}$ metric as a function of the number of stochastic forward passes of MC dropout for Ro-En and Et-En.}
\label{fig:forward_passes}
\end{figure}

% Table \ref{tab:dropout_forward_passes} shows the correlation for $\mathrm{D\mbox{-}TP}$ with $N \in \{10,20,30,40,50\}$ forward passes. We conclude that 30 forward passes is the best trade-off between cost and accuracy.%\mf{I am computing this for all language pairs to try and show a nice plot. }\todo{LS: in any case we should show only Pearson as we do not show Spearman elsewhere}
% \begin{table}[h]
% \begin{center}
% \begin{tabular}{|l | c |} 
% \hline
% & $r$ \\ % & $r_s$ \\ 
% \hline%
%$\mathrm{D\mbox{-}TP_{50}}$ & 0.524 \\ % & 0.552 \\
%$\mathrm{D\mbox{-}TP_{40}}$ & 0.522 \\ % & 0.553 \\
%$\mathrm{D\mbox{-}TP_{30}}$ & 0.544 \\ % & 0.553 \\
%$\mathrm{D\mbox{-}TP_{20}}$ & 0.512 \\ % & 0.549\\
%$\mathrm{D\mbox{-}TP_{10}}$ & 0.516 \\ % & 0.549 \\
%$\mathrm{D\mbox{-}TP_{5}}$ & 0.490 \\ % & 0.541 \\
%\hline
%\end{tabular}
%\end{center}
%\caption{Pearson ($\rho$) correlation between the mean of predictive probabilities computed with model parameters perturbed by MC dropout with different number of inference passes.}
%\label{tab:dropout_forward_passes}
%\end{table} 

% This result is interesting as it relates to the issue of linguistic variation in translation, widely discussed in relation to reference-based MT evaluation.

\paragraph{Group III} While our attention-based metrics also achieve a sensible correlation with human judgments, it is considerably lower than the rest of the unsupervised indicators. On the one hand, attention may not provide enough information to be used as a quality indicator of its own, since 
there is no direct mapping between words in different languages, and, therefore, high entropy in attention weights does not necessarily indicate low translation quality. We leave experimentation with combining attention and probability-based measures to future work.

On the other hand, the use of multi-head attention with multiple layers in Transformer may negatively affect the results. As shown by \citet{voita2019analyzing}, different attention heads in Transformer are responsible for different functions. Therefore, combining the information coming from different heads and layers in a simple way may not be an optimal solution. To test whether this is the case, we computed attention entropy\footnote{When computing entropy, we exclude end of sentence ``EOS'' mark, as it is not a real word, and renormalize the remaining attention weights.} for all possible combinations of heads and layers. Results are shown in Table \ref{tab:uncertainty_indicators} ($\mathrm{AW\mbox{:}\text{best head/layer}}$). Indeed, for all language pairs the best head/layer combination significantly outperforms other attention-based measurements suggesting that this method should be preferred over simple averaging. Using the best head/layer combination for QE is limited by the fact that it requires validation on a dataset annotated with DA. This outcome opens an interesting direction for further experiments to automatically discover the best possible head/layer combination. %\paco{I find this last part problematic because we claim to use unsupervised methods, yet we had to use data to choose the best attention layer.}\mf{I tried to reformulate this bit above}
% \footnote{We found that for all language pairs attention head with the best correlation comes from the lower layers of encoder-decoder mechanism. It is consistent with the idea that different layers play different roles in the attention mechanism \cite{voita2019analyzing,raganato2018analysis}. \citet{raganato2018analysis} suggest that self-attention focus on local dependencies in lower layers and finds long dependencies on higher layers. \mf{Can we explain what roles they play in one sentence here? Otherwise we should remove this.}}   
% There may be several reasons for that. On the one hand, it may be due to the fact that there is no direct mapping between words in different languages, %for example, Estonian word ``üksteist'' means ``each other''
% and, therefore, high entropy in attention weights does not necessarily indicate low translation quality. On the other hand, \citet{voita2019analyzing} showed that different heads from different layers are responsible for different functions: positional, syntactic and rare words. They analysed self-attention, but encoder-decoder likely follows a similar pattern. If this is the case, combining the information coming from different heads and layers in a simple way may not be an optimal solution and, as can be seen from Table \ref{tab:uncertainty_indicators}, averaging and taking the maximum give worse results compared to the result of the best head-layer.  To choose the best head-layer we have computed entropies for all heads and we have observed the huge difference in correlation coefficients across all heads, for example, the highest value of Pearson correlation coefficient for Estonian-English is almost 2.5 times higher than the smallest one. Also, we have noticed for all language pairs the head showed the best correlation comes from the lower layers of encoder-decoder mechanism. It is consistent with the idea that different layers play different roles in the attention mechanism \cite{voita2019analyzing,raganato2018analysis}.

\input{figures/distribution_across_languages.tex}
% \input{figures/metrics_scatter.tex}


==> experiments_short.tex <==
\section{Experiments and Results}
\label{sec:experiments}
Below we analyse how our unsupervised QE indicators correlate with human judgments.

\subsection{Settings}

% \paragraph{Data}
\textbf{Data.}
We use the dataset and NMT models described in \S \ref{subsec:data}. To make the results comparable to supervised QE, we use the test (1K) partition of the dataset for evaluation, whereas train (7K) and dev (1K) are used to train the supervised QE system.

\paragraph{Benchmark systems}
%\textbf{Benchmark systems.}
We compare the performance of the proposed unsupervised QE measures against the best performing approach to supervised QE with available open-source implementation, namely the Predictor-Estimator architecture~\cite{kim2017predictor} provided by OpenKiwi toolkit ~\cite{openkiwi}. % This model is an encoder-decoder RNN ({\it predictor}), which predicts words along with context representation from an attention mechanism. These representations are used as input for a unidirectional RNN ({\it estimator}) that produces quality estimates. We trained a Predictor model on the same data as the NMT systems, while the Estimator model was trained on the 7K DA judgement data. % (see Section~\ref{subsec:data}). %For each of the two models, we used the default training configuration provided by~\citet{openkiwi}.

As another point of comparison, we compute popular reference-based evaluation metrics: BLEU \cite{papineni2002bleu,Lin:2004orange}, Meteor \cite{denkowski2014meteor}, TER \cite{snover2006study} and ChrF \cite{popovic:2015:WMT2015}, for Estonian-English, for which we have independently collected reference translations. % (see Section \ref{subsec:data}).

\input{tables/summary_table_all_languages_pearson}

\subsection{Correlation with Human Judgments}

Table \ref{tab:uncertainty_indicators} shows Pearson correlation with DA for the unsupervised QE indicators described in \S \ref{sec:unsupervised_quality_estimation}, as well as for the supervised QE system and the reference-based metrics presented above. Unsupervised QE indicators are further grouped as follows: \textbf{Group I} corresponds to the measurements obtained with standard decoding (\S \ref{subsec:probability}); \textbf{Group II} contains indicators computed using MC dropout (\S \ref{subsec:uncertainty});\footnote{We use dropout rate of 0.3 and apply dropout before each weight layer. We perform $N=30$ inference passes to obtain posterior probability distribution for estimating model uncertainty.} and
\textbf{Group III} contains the results for attention-based indicators (\S \ref{subsec:attention}). We use Hotelling-Williams test to compute significance of the difference between dependent correlations \cite{Williams:1959} with p-value $< 0.05$. Results that are not significantly outperformed by any method are underlined; results that are not significantly outperformed by any other method from the same group are marked in bold.

\begin{figure*}[ht]
\centering
\begin{subfigure}  
    \includegraphics[width=0.45\textwidth]{figures/token-probas_seg19.png}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.45\textwidth]{figures/token-probas_seg313.png}
\end{subfigure}
\caption{High-quality (left) and low-quality (right) Estonian-English translations with very similar overall sentence-level probability (-0.50 and -0.48 for the first and second sentence, respectively) but very different patterns in the sequence of token-level probabilities.}
\label{fig:token_probabilities}
\end{figure*}

\input{tables/example_variation_v2.tex}

We observe that the simplest measure that can be extracted from NMT, sequence-level probability ($\mathrm{TP}$), already performs competitively, in particular for the medium-resource language pairs. $\mathrm{TP}$ is consistently outperformed by $\mathrm{D\mbox{-}TP}$ indicating that NMT output probabilities are not perfectly calibrated. This outcome confirms our hypothesis that estimating model uncertainty improves correlation with perceived translation quality. Furthermore, our unsupervised approach outperforms current SOTA in supervised QE. These results position the proposed unsupervised QE methods as an attractive alternative to the supervised approach.%, as they can be extracted as a by product of translation with no need to access any additional resources besides the NMT system itself. 

For both unsupervised and supervised methods performance varies considerably across language pairs. The highest correlation is achieved for the medium-resource languages, whereas for high-resource languages it is drastically lower. The main reason for this difference is a lower variability in translation quality.% for high-resource language pairs.
Figure \ref{fig:distribution_across_languages} shows the %the distribution of DA scores and
scatter plots for Romanian-English, which has the best correlation results, and English-German with the lowest correlation for all quality indicators. Romanian-English contains a substantial number of high-quality sentences, but the rest of the translations are uniformly distributed across the quality range. The distribution for English-German is highly skewed, as the vast majority of the translations are of high quality. In this case capturing meaningful variation appears to be more challenging, as the differences reflected by the DA may be more subtle than any of the QE methods is able to reveal. % \paco{It is interesting that here we're seeing the opposite effect as with the WMT datasets.}

The reason for a lower correlation for Sinhala and Nepalese is different. For unsupervised indicators it can be due to the difference in model capacity\footnote{Models for these languages were trained using Transformer-Big architecture from \citet{vaswani2017attention}.} 
%Transformer for the rest of the language pairs)\mf{Vishrav, could you please confirm this?}
and the amount of training data. On the one hand, as demonstrated by \citet{guo2017calibration}, increasing depth and width of the model may negatively affect calibration. On the one hand, due to the small amount of training data the model can overfit producing inferior results in terms of both translation quality and correlation. It is noteworthy, however, that supervised QE system suffers a larger drop in performance, % than unsupervised indicators
as its predictor component requires large amounts of parallel data for successful training. We suggest, therefore, that unsupervised QE is more stable in low-resource scenarios than supervised approaches. 

We now look in more detail at the three groups of unsupervised measurements in Table \ref{tab:uncertainty_indicators}.

\paragrph{Group I}
% \textbf{Group I.}
Average entropy of the softmax output ($\mathrm{Soft\mbox{-}Ent}$) and dispersion of the values of token-level probabilities ($\mathrm{Sent\mbox{-}Var}$) achieve a significantly higher correlation than TP metric for four language pairs. 
% produce competitive results, with a substantial improvement over sequence-level translation probability for some of the language pairs.
$\mathrm{Soft\mbox{-}Ent}$ captures uncertainty of the output probability distribution, which appears to be a more accurate reflection of the overall translation quality. $\mathrm{Sent\mbox{-}Var}$ captures a pattern in the sequence of token-level probabilities that helps detect low-quality translation illustrated in Figure \ref{fig:token_probabilities}. Figure \ref{fig:token_probabilities} shows two translations from Estonian into English that have the absolute DA scores of 62 and 1, respectively, the first sentence being clearly superior in quality. But the difference in their sentence-level log-probability is negligible: -0.50 and -0.48 for the first and second translations, respectively. By contrast, the sequence of token-level probabilities for these two sentences looks very differently, as the second sentence has larger variation in the log-probabilities for adjacent words, with very high probabilities for high-frequency function words and low probabilities for content words. %\todo{LS: this is another candidate to go if we need space as I'm not sure it adds much to the paper, even though it's super interesting. we may be able to explain without plots} %We suggest that further analysis of the patterns of token-level probabilities in translated sequences can lead to even better correlation results.

\paragraph{Group II}
%\textbf{Group II.}
The best results are achieved by the $\mathrm{D\mbox{-}TP}$ metric. % that measures the expectation over posterior probabilities obtained using MC dropout. %This confirms our hypothesis that a better representation of model uncertainty leads to a higher correlation with human judgements of MT quality. 
Interestingly, $\mathrm{D\mbox{-}Var}$ has a much lower correlation, since by only capturing variance it ignores the actual probability estimate assigned by the model to the given output.\footnote{This is in contrast with the work by \citet{wang2019improving} where D-Var is one of the best performing metric for NMT training with back-translation, demonstrating an essential difference with the QE task.}

Table \ref{tab:linguistic_variation} provides an illustration of how model uncertainty captured by MC dropout reflects the quality of MT output. The first example contains a low quality translation, with a high variability in MT hypotheses obtained with MC dropout. By contrast, MC dropout hypotheses for the second high-quality example are very similar and in fact constitute valid linguistic paraphrases of each other. This fact is directly exploited by our $\mathrm{D\mbox{-}Lex\mbox{-}Sim}$ metric that measures the variability between MT hypotheses generated with perturbed model parameters and performs on pair with $\mathrm{D\mbox{-}TP}$. $\mathrm{D\mbox{-}Lex\mbox{-}Sim}$, besides capturing model uncertainty, reflects the potential complexity of the source segments, as the number of different possible translations of the sentences is an indicator of its inherent ambiguity. %It should be noted, however, that this is a less practical method, since generating additional translations is more costly than re-scoring an already generated MT output multiple times.

% A question that arises for the practical application of $\mathrm{D\mbox{-}TP}$ is how the results would be affected by the number of stochastic forward passes. Figure \ref{fig:forward_passes} shows Pearson correlation with human judgments for our $\mathrm{D\mbox{-}TP}$ metric as a function of the number of stochastic forward passes of MC dropout for Romanian-English and Estonian-English, where this metric brings the largest gains over sequence-level probability. Based on the results in Figure \ref{fig:forward_passes}, we suggest using $N=20$ as increasing N beyond 20 does not give any improvement in correlation.

% \begin{figure}[ht]
%\centering
%     \includegraphics[width=0.45\textwidth]{figures/n_forward_passes.png}
% \caption{Pearson correlation with human judgments for our $\mathrm{D\mbox{-}TP}$ metric as a function of the number of stochastic forward passes of MC dropout for Ro-En and Et-En.}
% \label{fig:forward_passes}
% \end{figure}

\paragraph{Group III}
%\textbf{Group III.}
While our attention-based metrics also achieve a sensible correlation with human judgments, it is considerably lower than the rest of the unsupervised indicators. On the one hand, attention may not provide enough information to be used as a quality indicator of its own, since 
there is no direct mapping between words in different languages, and, therefore, high entropy in attention weights does not necessarily indicate low translation quality. We leave experimentation with combining attention and probability-based measures to future work.

On the other hand, the use of multi-head attention with multiple layers in Transformer may negatively affect the results. % As shown by \citet{voita2019analyzing}, different attention heads are responsible for different functions. Therefore, combining the information coming from different heads and layers in a simple way may not be an optimal solution.
To test whether this is the case, we calculated attention entropy %\footnote{When computing entropy, we exclude end of sentence ``EOS'' mark, as it is not a real word, and renormalize the remaining attention weights.}
for all possible combinations of heads and layers and computed the correlation with DA judgments. Results are shown in Table \ref{tab:uncertainty_indicators} ($\mathrm{AW\mbox{:}\text{best head/layer}}$). Indeed, for all language pairs the best head/layer combination significantly outperforms other attention-based measurements suggesting that this method should be preferred over simple averaging. Using the best head/layer combination for QE is limited by the fact that it requires validation on a dataset annotated with DA. This outcome opens an interesting direction for further experiments to automatically discover the best possible head/layer combination. 

\input{figures/distribution_across_languages.tex}


==> figures/metrics_scatter.tex <==
\begin{figure*}
\centering
\begin{subfigure}
    \includegraphics[width=0.3\textwidth]{figures/metrics-scatter/sien_tp.png}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.3\textwidth]{figures/metrics-scatter/roen_tp.png}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.3\textwidth]{figures/metrics-scatter/ende_tp.png}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.3\textwidth]{figures/metrics-scatter/sien_soft-ent.png}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.3\textwidth]{figures/metrics-scatter/roen_d-tp.png}
\end{subfigure}
\begin{subfigure}
    \includegraphics[width=0.3\textwidth]{figures/metrics-scatter/ende_sent-var.png}
\end{subfigure}
\label{fig:distribution_across_languages}
\caption{Scatter plots for Sinhala-English, Romanian-English and German-English showing the relation between DA judgments and TP (top) vs. DA judgments and best performing metrics for each language pair (bottom)}
\end{figure*}


==> introduction.tex <==
\section{Introduction}

% {\bf Niko's comments: }

% 1. Main selling point is Unsupervised QE using info from an (already trained) NMT model. This should be highlighted more and become more clear.

% 2. I would suggest the following structure:
 
%  - Para 1: Advances in NMT, used in many practical applications. Problems of NMT: (1) not consistent across languages/domains/data; (2) might be deceptive by generating fluent translations; and (3) models might be  overconfident. Therefore, having a mechanism to inform the users to what extent should trust NMT models is crucial!  

% - Para 2: QE. What is QE. Definition on the word level/sentence level (note that here we focus on sentence level), refs to seminal previous work. Why is it useful? Limitations of current QE models.

% - Para 3: In this paper, we are going to tackle QE and NMT limitations in one go! How? By using info from already trained NMT models that currently has been disregarded. What info? Uncertainty. Introduce what it is (refs to ML papers), what has been done in MT and uncertainty calibration and what you're going to do is different (they tried to tackle the problem of overconfidence but not QE, the one we're tackling here). If that's long (probably it will) split into two paragraphs after the introduction of what uncertainty is.

% - Para 4: What are the main contributions of the paper (we can use a bullet point list to begin with and decide to flatten it later if there are space requirements)

% 3. In general, you introduce a lot of stuff in the intro that might actually go to Background/Related work.

With the advent of neural models, Machine Translation (MT) systems have made substantial progress, reportedly achieving near-human translation quality under certain conditions \cite{hassan2018achieving,barrault2019findings}. %\todo{cite original Microsoft paper that claims that?}
MT is used in an increasing number of applications, with more users relying on it for practical needs. However, the quality of MT is still not consistent across language pairs, domains and datasets. Furthermore, neural MT (NMT) systems can be deceptive as they are able to generate fluent translations that are  different in  meaning from the original  \cite{bentivogli2016neural,castilho2017neural}.
In this context, having a mechanism to predict and inform the user on the extent to which a given MT output can be trusted or relied upon becomes crucial.

Quality estimation (QE) is an active field of research where the goal is to predict MT quality at test time when no gold standard human translation is available to be used for comparison. Influential MT evaluation campaigns, such as the WMT conference, have been benchmarking QE system submissions every year since 2012. Current neural-based QE systems have  been shown to provide highly accurate predictions of MT quality \cite{kim-lee-na:2017:WMT,fonseca2019findings}. However, such systems %are resource-heavy and 
require large amounts of parallel data for pretraining, as well as in-domain translations annotated with quality labels for training. 
%In fact, neural-based QE systems and NMT use similar architectures and training procedures, and therefore current approaches to QE suffer from  some of the main issues in NMT, such as a drastic decrease in performance for out-of-domain data and in low-resource settings.

As an alternative, in this paper we explore unsupervised approaches to QE. We posit that NMT models offer a rich source of information on translation quality that has been so far disregarded in the work on QE for NMT outputs.
%
Translation probabilities and language model probabilities have been  used as  indicators of model confidence to predict translation quality for statistical MT systems \cite{specia2013quest,blatz2004confidence} in feature-based QE approaches along with many other indicators. NMT systems have however been treated as a black box. Neural-based QE approaches ignore model-specific information. This is due, on the one hand, to the complexity of the underlying NMT models. On the other hand, as has been shown in the recent work \cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple}, despite remarkable success in a wide variety of machine learning tasks, deep neural networks are not well calibrated and produce overconfident predictions.

We test these observations in the first attempt to use several model-internal NMT information as quality predictors. We study how the reliability of NMT model predictive probabilities changes depending on model architecture, search algorithm and the extent of training. Different from the few existing work on calibration in NMT \cite{ott2018analyzing,kumar2019calibration}, we collect human judgments of translation quality for this analysis. %We show that some of the models commonly used in practice produce reliable confidence estimates. % The models and the data produced for this study will be made publically available.

In addition to {\em model confidence}, we propose to study {\em model uncertainty}. %which can be seen as a way of improving the reliability NMT model confidence estimates based on uncertainty quantification methods for deep Neural Networks (NNs). 
%\todo{define confidence/uncertainty: model/epistemic uncertainty vs aleatoric or input/output uncertainty}
Uncertainty in deep learning typically relies upon Bayesian NNs \cite{tran2019bayesian} that learn a distribution over model parameters and use it to represent model uncertainty (also called {\em epistemic uncertainly}). This type of uncertainty captures our lack of information about the underlying model that generated the training data \cite{kendall2017uncertainties}. %However, Bayesian NNs require significant changes in the training procedure and may involve prohibitive computational costs. A few methods have been recently developed to allow for approximate Bayesian inference with minor changes to the training pipeline \cite{gal2016dropout}. 
To avoid changing the training procedure in NMT, which has proved successful, we explore various approximations for uncertainty quantification, e.g. \cite{gal2016dropout}, which are based on the idea of model  calibration\todo{Marina to check this}. % and leverage the improved confidence estimates to predict translation quality.

We hypothesize that if we can estimate NMT model uncertainty,  
%(e.g. translation probabilities produced by the NMT model are well calibrated), 
this will strongly correlate with the perceived quality of generated translations.  
%
To that end, we devise a set of unsupervised quality indicators that can be produced as a by-product of NMT decoding. 

Finally, besides softmax probability distribution, we also use attention mechanism to extract information on model confidence \todo{confidence or uncertainty - maybe move earlier}. 
%Attention weights have been used for confidence estimation in RNN-based NMT \cite{rikters2017confidence}. 
Previous studies have analysed the interpretability of attention in Transformer models \cite{vaswani2017attention}, however, none of them considers attention as a source of information on model confidence    \cite{voita2019analyzing, vig2019analyzing}. %This is the first attempt to explore attention in state-of-the-art Transformer models, as it involves a more complex attention mechanism.  
%Apart from few approaches that use attention weights to estimate word-level confidence for recurrent NNs (see Section \ref{related_work}), %\mf{Maybe we should formulate contributions in a bullet-point list?}

Our {\bf main contributions} are as follows: (i) The first investigation on NMT model confidence and uncertainty on several NMT variants for the purposes of unsupervised QE;\todo{add ref to section} (ii) New uncertainty-aware indicators from NMT models and a thorough evaluation on how they correlate with human judgments of translation quality; (iii) The first  attempt at analysing the attention distribution for the purposes of unsupervised QE in Transformer models; (iv) A new dataset with 6 language pairs, machine translations by various NMT models and human judgements of quality. \textcolor{blue}{Our results suggest that unsupervised QE indicators computed from well-calibrated NMT internal model information can outperform state-of-the-art supervised QE approaches when the quality distribution of the NMT translations is not too skewed.}      
We note that while the paper covers QE at sentence level, the extension of our unsupervised metrics to word-level QE would be straightforward.

% Neural MT systems generate a probability distribution over language vocabulary for each generated target word. We suggest that well calibrated predictive probabilities from the MT model are strongly correlated with the quality of generated translations. 

% Due to non-linearity and complexity of the functions, NNs are poor at quantifying uncertainty.

% One such approach called Monte Carlo dropout \cite{gal2016dropout} consists in using dropout at test time. Due to its simplicity, this method has been successfully applied to a variety of machine learning tasks \cite{dong2018confidence,miok2019prediction,wang2019improving}.

% if a neural MT model is capable of representing uncertainty, its predictive probabilities will be a good indicator of translation quality.

% Very few studies have looked at model uncertainty in the MT task \cite{ott2018analyzing}. Neural MT translation have achieved very good results, but its performance is not stable, as it can produce near human quality translations but also nonsensical results. Moreover, such models can generate well-formed sentences in the target language, which completely distort the meaning of the source. In this context, quality estimation gains particular importance, as it can inform the user to what extent they can trust a particular translation. 

% In this paper, we propose to look at unsupervised quality indicators to improve on the above issues, as well as increase the interpretability of neural MT models. On the one hand, we leverage the information that can be extracted from the neural MT model itself in order to produce quality estimates. On the other hand, we look at cross-lingual representation thus addressing QE as a cross-lingual similarity task.



==> introduction_v2.tex <==
\section{Introduction}

With the advent of neural models, Machine Translation (MT) systems have made substantial progress, reportedly achieving near-human translation quality for high-resource language pairs \cite{hassan2018achieving,barrault2019findings}. MT is used in an increasing number of applications, with more users relying on it for practical needs. However, the quality of translations provided by state-of-the-art MT systems is still not consistent across language pairs, domains and datasets. Furthermore, neural MT (NMT) systems can sometimes be deceptive to the end user as they are able to generate fluent translations that are different in meaning from the original \cite{bentivogli2016neural,castilho2017neural}.
In this context, having a mechanism to predict and inform the user on what extent a given MT output can be trusted or relied upon becomes crucial.

Quality estimation (QE) is an active field of research where the goal is to predict the quality of the output provided by an MT system at test time when no gold standard human translation is available to be used for comparison. Influential MT evaluation campaigns, such as the WMT conference, have been benchmarking QE system submissions every year since 2012. Current neural-based QE systems have been shown to provide highly accurate predictions of MT quality \cite{kim-lee-na:2017:WMT,fonseca2019findings}. However, such systems %are resource-heavy and 
require large amounts of parallel data, as well as in-domain translations annotated with quality labels for training the models. 
%In fact, neural-based QE and NMT systems use similar architectures and training procedures, and therefore current approaches to QE suffer from some of the main issues in NMT, such as a decrease in performance for out-of-domain data and in low-resource settings. 
Output probabilities from translation and language models have been used to represent model confidence and predict translation quality for statistical MT systems \cite{specia2013quest,blatz2004confidence} in feature-based QE approaches along with many other indicators. Yet, NMT systems have been treated as a black box. Even neural-based QE approaches ignore internal model information. \paco{Sentence to justify why that is important} %\shuo{I'm a bit confused here. What kind of model-specific information is ignored?}

%As an alternative, 
In this paper we posit that encoder-decoder NMT models \cite{sutskever2014sequence,bahdanau2014neural,luong2015effective,vaswani2017attention} offer a rich source of information on translation quality that has been so far disregarded in the work on QE for NMT outputs. %NMT is based on encoder-decoder neural networks with attention mechanism \cite{sutskever2014sequence,bahdanau2014neural,luong2015effective,vaswani2017attention}. 
%We show that even taking sentence-level translation probabilities of top hypotheses %the top translation hypothesis in these systems 
%provides a simple way for obtaining a confidence estimate, and  
%, which can be used to predict output quality. Besides this simple strategy, we
Importantly, such information allows for {\bf unsupervised approaches to QE} of NMT systems. We
We devise methods that leverage %and summarize softmax 
the probability distribution for each generated token to obtain sentence-level measurements of confidence. 
It has been shown that output probabilities from deep neural networks, if well \emph{calibrated}, are reliable predictors  \cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple}. 
%Interpretability of attention mechanism in Transformer models has been the focus of a particular interest in recent work \cite{voita2019analyzing, vig2019analyzing}. However, none of them considers attention for the purposes of QE. 
\paco{This sentence is core to the contribution of the paper, yet doesn't sound novel enough given that similar approaches have been tried to filter backtranslation}.
%Although, as will be shown in this paper, above measurements already provides competitive results for QE, 
 % we argue that output probabilities from deep neural networks are not well \emph{calibrated} \cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple} (i.e. not always representative of the true translation likelihood) and
We hypothesize that better estimation of uncertainty in NMT will lead to stronger correlation with the quality of generated translations. Uncertainty quantification in deep learning typically relies on Bayesian formalism \cite{mackay1992bayesian,graves2011practical,welling2011bayesian,gal2016dropout,tran2019bayesian}. 
%\todo{LS: this is still confusing: is calibration and quantification the same thing then?}\mf{Moved the sentence about calibration to the next paragraph.} 
Bayesian neural networks learn a posterior distribution over parameters that quantifies \emph{epistemic} uncertainty, i.e. our lack of knowledge as to which model generated the training data.\footnote{A distinction is typically made between epistemic and aleatoric uncertainty, where the latter captures the noise inherent to the observation \cite{kendall2017uncertainties}. We leave modelling aleatoric uncertainty in NMT for future work.} To avoid changing the NMT training procedure, instead of using Bayesian networks we explore various approximations that can be applied at inference time, such as Monte Carlo dropout 
%, a popular approximation to Bayesian inference developed by 
\citet{gal2016dropout} 
to devise a set of unsupervised quality indicators with better quantification of model uncertainty. 
%that can be obtained as a by-product of translation and can be extracted from any encoder-decoder NMT model. 
Finally, we also suggest that the attention mechanism constitutes another interesting source of information for unsupervised QE.


It has been shown that factors such as training settings, search algorithms, network architecture can negatively affect model calibration \cite{guo2017calibration,ott2018analyzing}, i.e. the extent to which predictive probabilities are representative of the likelihood that the generated translation is correct. We conduct experiments to study how the reliability of NMT predictive probabilities changes depending on these factors. %Different from the few existing work on calibration in NMT \cite{ott2018analyzing,kumar2019calibration}, we collect human judgments of translation quality for this analysis. 
We note that while the paper covers QE at sentence level, the extension of our unsupervised metrics to word-level QE would be straightforward.

Our {\bf main contributions} are as follows: (i)  A new dataset with six language pairs, 10K machine translations per language by various NMT models and human judgements of quality (Section \ref{subsec:data}); (ii) A set of new unsupervised quality indicators that can be produced as a by-product of NMT decoding and a thorough evaluation on how they correlate with human judgments of translation quality (Sections \ref{sec:unsupervised_quality_estimation} and \ref{sec:experiments}); (iii)  The first attempt at analysing the attention distribution for the purposes of unsupervised QE in Transformer models (Sections \ref{sec:unsupervised_quality_estimation} and \ref{sec:experiments}); (iv) The first investigation on NMT model  uncertainty on several NMT variants for the purposes of unsupervised QE (Section  \ref{subsec:results_uncertainty_models}). Our results suggest that unsupervised QE indicators computed from well-calibrated NMT model information can outperform state-of-the-art supervised QE approaches when the quality distribution of the NMT translations is not too skewed.

%As an alternative, in this paper we explore unsupervised approaches to QE for NMT systems. We posit that NMT models offer a rich source of information on translation quality that has been so far disregarded in the work on QE for NMT outputs. NMT systems generate a probability distribution over target vocabulary and a likely output sequence is selected typically using beam search. Sequence-level probability can be interpreted as model confidence for a given translation output. We devise a set of measures that capture model confidence based on the softmax probability distribution to predict translation quality in a fully unsupervised manner. 

%However, as has been shown in the recent work \cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple}, despite remarkable success in a wide variety of machine learning tasks, output probability from deep neural networks may be poorly \emph{calibrated}, i.e. they are not representative of the true likelihood of correctness tending towards overconfidence. We test these observations in the first attempt to use model-internal NMT information to predict quality. We study how the reliability of NMT model predictive probabilities changes depending on model architecture, search algorithm and the extent of training. Different from the few existing work on calibration in NMT \cite{ott2018analyzing,kumar2019calibration}, we collect human judgments of translation quality for this analysis.

%Although, as will be shown in this paper, using confidence estimates extracted from NMT already provide competitive results for QE, we hypothesize that if we can better estimate NMT model uncertainty, a higher correlation with human judgments can be achieved. In deep learning uncertainty quantification typically relies on the Bayesian formalism \cite{mackay1992bayesian,graves2011practical,welling2011bayesian,gal2016dropout,tran2019bayesian}. Bayesian neural networks learn a posterior distribution over parameters that quantifies \emph{epistemic} uncertainty, i.e. our lack of knowledge as to which model generated the training data.\footnote{A distinction is typically made between epistemic and aleatoric uncertainty, where the latter captures the noise inherent to the observation \cite{kendall2017uncertainties}. We leave experiments with aleatoric uncertainty for NMT to future work.} To avoid changing the training procedure in NMT, which has proved successful, we explore various methods that only require changes at inference time, such as a non-Bayesian temperature scaling approach \cite{platt1999probabilistic} and Monte Carlo dropout, a popular approximation to Bayesian inference developed by \citet{gal2016dropout}.

%Finally, besides softmax probability distribution, we use attention mechanism \cite{bahdanau2014neural,vaswani2017attention} as a source of information on translation quality. Previous studies have analysed the interpretability of attention in Transformer models \cite{vaswani2017attention}, however, none of them considers attention as a source of information on model confidence \cite{voita2019analyzing, vig2019analyzing}.


==> introduction_v3.tex <==
\section{Introduction}

With the advent of neural models, Machine Translation (MT) systems have made substantial progress, reportedly achieving near-human translation quality for high-resource language pairs \cite{hassan2018achieving,barrault2019findings}. MT is used in an increasing number of applications, with more users relying on it for practical needs. However, the quality of translations provided by state-of-the-art MT systems is still not consistent across language pairs, domains and datasets. Furthermore, neural MT (NMT) systems can sometimes be deceptive to the end user as they are able to generate fluent translations that are different in meaning from the original \cite{bentivogli2016neural,castilho2017neural}.
In this context, having a mechanism to predict and inform the user on what extent a given MT output can be trusted or relied upon becomes crucial.

Quality estimation (QE) aims to predict the quality of the output provided by an MT system at test time when no gold standard human translation is available to be used for comparison. 
%Influential MT evaluation campaigns, such as the WMT conference, have been benchmarking QE system submissions every year since 2012. 
State-of-the-art QE models use supervised neural-based learning algorithms, requiring large amounts of parallel data for pre-training as well as in-domain translations annotated with quality labels for training \cite{kim-lee-na:2017:WMT,fonseca2019findings}. 

% In this paper we propose to treat QE as an {\bf unsupervised problem}. We posit that encoder-decoder NMT models \cite{sutskever2014sequence,bahdanau2014neural,luong2015effective,vaswani2017attention} offer a rich source of information on translation quality that has been so far disregarded in the work on QE for NMT outputs. We explore attention mechanism and NMT model probability distribution to devise a set of metrics that can be extracted as a by-product of translation.

In this paper we posit that encoder-decoder NMT models \cite{sutskever2014sequence,bahdanau2014neural,luong2015effective,vaswani2017attention} offer a rich source of information on translation quality that has been so far disregarded in the work on QE for NMT outputs. We propose, therefore, to treat QE as an {\bf unsupervised problem}. To achieve this, we study output probability distribution in NMT systems. Probabilities in a well calibrated model correspond to the empirical likelihood of the predictions. In the context of MT, we expect that model confidence estimates, if well calibrated, should reliably predict the quality of MT output.

However, it has been shown that output probabilities from deep neural networks are not generally well calibrated % \emph{calibrated}
\cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple}. %, i.e. not always representative of the % true translation likelihood 
% true likelihood of the predictions
%\paco{This sentence is core to the contribution of the paper, yet doesn't sound novel enough given that similar approaches have been tried to filter backtranslation}.
We hypothesize that better estimation of uncertainty in NMT will lead to stronger correlation with the perceived quality of generated translations. % and thus will this can be a good unsupervised quality predictors.
Uncertainty quantification in deep learning typically relies on Bayesian formalism \cite{mackay1992bayesian,graves2011practical,welling2011bayesian,gal2016dropout,tran2019bayesian}. Bayesian neural networks learn a posterior distribution over parameters that quantifies \emph{epistemic} uncertainty, i.e. our lack of knowledge as to which model generated the training data.\footnote{A distinction is typically made between epistemic and aleatoric uncertainty, where the latter captures the noise inherent to the observation \cite{kendall2017uncertainties}. We leave modelling aleatoric uncertainty in NMT for future work.} To avoid changing the NMT training procedure, instead of using Bayesian networks we explore various approximations that can be applied at inference time, such as Monte Carlo dropout \cite{gal2016dropout}. 

%As result, we devise a set of unsupervised quality indicators. % based on quantification of model uncertainty. 
% Different from existing work on calibration in NMT \cite{ott2018analyzing,kumar2019calibration} that defines translation correctness by comparison to a human translation, we collect {\em human judgments} of translation quality at the sentence level and use correlation between these and our indicators for evaluation. %To evaluate the proposed indicators 
To test our hypothesis and design an  approach to QE without supervision we devise a set of measurements that can be extracted from an NMT model based on softmax probability distributions, these distributions with uncertainty quantification, and the distribution of attention weights. To evaluate our approach, we create a new dataset with six language pairs, 10K machine translations per language by SOTA NMT models and multiple {\em direct assessment} (DA) \cite{da_paper} human judgements of quality at the sentence level. 

% Finally, we examine the entropy of attention weights as another source of information for unsupervised QE.

Our {\bf main contributions} can be summarised as follows: (i) A new, large-scale dataset for sentence-level QE annotated with DA rather than post-editing metrics (Section \ref{subsec:data}); (ii) A set of unsupervised quality indicators that can be produced as a by-product of NMT decoding and a thorough evaluation on how they correlate with human judgments of translation quality (Sections \ref{sec:unsupervised_quality_estimation} and \ref{sec:experiments}); (iii)  The first attempt at analysing the attention distribution for the purposes of unsupervised QE in Transformer models (Sections \ref{sec:unsupervised_quality_estimation} and \ref{sec:experiments}); (iv) The first investigation on how model confidence relates to translation quality for different NMT architectures (Section  \ref{sec:discussion}). 

%It has been shown that factors such as training settings, search algorithms, network architecture can negatively affect model calibration \cite{guo2017calibration,ott2018analyzing}, i.e. the extent to which predictive probabilities are representative of the likelihood that the generated translation is correct. We conduct experiments to study how the reliability of NMT predictive probabilities changes depending on these factors.  
Our results suggest that unsupervised QE indicators computed from well-calibrated NMT model information can outperform state-of-the-art supervised QE approaches when the quality distribution of the NMT translations is not too skewed.

%As an alternative, in this paper we explore unsupervised approaches to QE for NMT systems. We posit that NMT models offer a rich source of information on translation quality that has been so far disregarded in the work on QE for NMT outputs. NMT systems generate a probability distribution over target vocabulary and a likely output sequence is selected typically using beam search. Sequence-level probability can be interpreted as model confidence for a given translation output. We devise a set of measures that capture model confidence based on the softmax probability distribution to predict translation quality in a fully unsupervised manner. 

%However, as has been shown in the recent work \cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple}, despite remarkable success in a wide variety of machine learning tasks, output probability from deep neural networks may be poorly \emph{calibrated}, i.e. they are not representative of the true likelihood of correctness tending towards overconfidence. We test these observations in the first attempt to use model-internal NMT information to predict quality. We study how the reliability of NMT model predictive probabilities changes depending on model architecture, search algorithm and the extent of training. Different from the few existing work on calibration in NMT \cite{ott2018analyzing,kumar2019calibration}, we collect human judgments of translation quality for this analysis.

%Although, as will be shown in this paper, using confidence estimates extracted from NMT already provide competitive results for QE, we hypothesize that if we can better estimate NMT model uncertainty, a higher correlation with human judgments can be achieved. In deep learning uncertainty quantification typically relies on the Bayesian formalism \cite{mackay1992bayesian,graves2011practical,welling2011bayesian,gal2016dropout,tran2019bayesian}. Bayesian neural networks learn a posterior distribution over parameters that quantifies \emph{epistemic} uncertainty, i.e. our lack of knowledge as to which model generated the training data.\footnote{A distinction is typically made between epistemic and aleatoric uncertainty, where the latter captures the noise inherent to the observation \cite{kendall2017uncertainties}. We leave experiments with aleatoric uncertainty for NMT to future work.} To avoid changing the training procedure in NMT, which has proved successful, we explore various methods that only require changes at inference time, such as a non-Bayesian temperature scaling approach \cite{platt1999probabilistic} and Monte Carlo dropout, a popular approximation to Bayesian inference developed by \citet{gal2016dropout}.

%Finally, besides softmax probability distribution, we use attention mechanism \cite{bahdanau2014neural,vaswani2017attention} as a source of information on translation quality. Previous studies have analysed the interpretability of attention in Transformer models \cite{vaswani2017attention}, however, none of them considers attention as a source of information on model confidence \cite{voita2019analyzing, vig2019analyzing}.


==> introduction_v4.tex <==
\section{Introduction}

With the advent of neural models, Machine Translation (MT) systems have made substantial progress, reportedly achieving near-human translation quality for high-resource language pairs \cite{hassan2018achieving,barrault2019findings}. MT is used in an increasing number of applications, with more users relying on it for practical needs. However, the quality of translations provided by state-of-the-art MT systems is still not consistent across language pairs, domains and datasets. Furthermore, neural MT (NMT) systems can sometimes be deceptive to the end user as they are able to generate fluent translations that are different in meaning from the original \cite{bentivogli2016neural,castilho2017neural}.
In this context, having a mechanism to predict and inform the user on what extent a given MT output can be trusted or relied upon becomes crucial.

Quality estimation (QE) is an active field of research where the goal is to predict the quality of the output provided by an MT system at test time when no gold standard human translation is available to be used for comparison. State-of-the-art QE models use supervised neural-based learning algorithms, requiring large amounts of parallel data for pre-training as well as in-domain translations annotated with quality labels for training \cite{kim-lee-na:2017:WMT,fonseca2019findings}. In this paper we posit that encoder-decoder NMT models \cite{sutskever2014sequence,bahdanau2014neural,luong2015effective,vaswani2017attention} offer a rich source of information on translation quality that has been so far disregarded in the work on QE for NMT outputs. We propose, therefore, to treat QE as an {\bf unsupervised problem}.

%% Nikos: First two paragraphs are great! The next one (two) paragraph(s) should clearly describe our approach to Unsupervised QE. Try not to blend findings (e.g. "we suggest...") or taking a position on how well calibrated NMT systems might be. We say in the previous paragraph that we are going to use info only from the NMT model. The next paragraph should concisely describe that info.

\paragraph{NA's suggestion (remove):} To achieve this, we use information from (a) the \emph{output probability distribution} obtained by the NMT system (i.e. the probabilities obtained by applying the softmax function over the entire vocabulary in the target language); and (b) the \emph{attention mechanism} during decoding.

\paragraph{NA Output Probabilities (remove):} We first assume that the more confident the decoder the better the quality of the translation. Sequence-level probability of the top MT hypothesis has been used for confidence estimation in statistical MT \cite{specia2013quest,blatz2004confidence}, however the output probabilities from deep neural networks are not generally well calibrated, i.e. not always representative of the true likelihood of the predictions \cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple}. Softmax output probabilities tend to be overconfident resulting in assigning high probability to predictions that are far away from the training data \cite{gal2016dropout}. Therefore, we design various ways to exploit softmax output distribution beyond the probability of the top-1 prediction by exploring uncertainty quantification methods to obtain better probability estimates \cite{gal2016dropout,lakshminarayanan2017simple}.  

{\bf NA: after this paragraph go straight to explaining attention}


\paragraph{Original Version: } To achieve this, we explore output probability distribution in NMT. We suggest, however, that sequence-level probability of the top MT hypothesis that has been proposed for confidence estimation in statistical MT \cite{specia2013quest,blatz2004confidence}, is not the optimal solution to predict translation quality for NMT systems. It has been shown that output probabilities from deep neural networks are not generally well calibrated
\cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple}, i.e. not always representative of the true likelihood of the predictions. Softmax output probabilities tend to be overconfident resulting in high probability for predictions that are far away from the training data \cite{gal2016dropout}. We hypothesize, therefore, that better estimation of uncertainty in NMT will lead to stronger correlation with the perceived quality of generated translations. On the one hand, we design various ways to exploit softmax output distribution beyond the probability of the top-1 prediction. On the other hand, we explore uncertainty quantification methods to obtain better probability estimates \cite{gal2016dropout,lakshminarayanan2017simple}. 
% Predictive probabilities obtained by applying softmax function to the last neural layer of a neural network classifier tend to be overconfident resulting in high probability for predictions that are far away from the training data \cite{gal2016dropout}. We hypothesize, therefore, that better estimation of uncertainty in NMT will lead to stronger correlation with the perceived quality of generated translations. On the one hand, we design various ways to exploit softmax output distribution beyond the probability of the top-1 prediction. On the other hand, we explore uncertainty quantification methods to obtain better probability estimates \cite{gal2016dropout,lakshminarayanan2017simple}. 


%% Nikos: From here it gets clear again :)
In addition, we study attention mechanism as another source of information on NMT quality. Attention can be interpreted as soft alignment, providing an indication of the strength of relation between source and target words \cite{bahdanau2014neural}. While this interpretation is straightforward for Recurrent Neual Networks (RNN) \cite{rikters2017confidence}, its application to current state-of-the-art (SOTA) Transformer models with multi-head attention \cite{vaswani2017attention} is challenging. In this work, we analyse to what extent meaningful information on translation quality can be extracted from multi-head attention.

We note that the reliability of model probability estimates in neural networks can be affected by multiple factors, such as model architecture, training and search \cite{guo2017calibration}. To evaluate the performance of our unsupervised QE methods, we collect a new dataset for QE with 6 language pairs, multiple NMT models and 10K original segments per language pair. By contrast to the vast majority of work on QE that uses semi-automatic metrics based on post-editing distance as gold standard, we follow current best practices in MT evaluation and conduct a fully manual assessment of MT output quality based on direct assessment (DA) methodology \cite{da_paper}.

Our {\bf main contributions} can be summarised as follows: (i) A new, large-scale dataset for sentence-level QE annotated with DA rather than post-editing metrics (Section \ref{subsec:data}); (ii) A set of unsupervised quality indicators that can be produced as a by-product of NMT decoding and a thorough evaluation on how they correlate with human judgments of translation quality (Sections \ref{sec:unsupervised_quality_estimation} and \ref{sec:experiments}); (iii)  The first attempt at analysing the attention distribution for the purposes of unsupervised QE in Transformer models (Sections \ref{sec:unsupervised_quality_estimation} and \ref{sec:experiments}); (iv) The first investigation on how model confidence relates to translation quality for different NMT architectures (Section  \ref{sec:discussion}). Our results suggest that unsupervised QE indicators obtained from well-calibrated NMT model probabilities can outperform state-of-the-art supervised QE approaches when the quality distribution of the NMT translations is not too skewed.


==> neural_mt.tex <==
\section{Neural Machine Translation}
\label{subsec:neuralmt}

\todo{LS: summarise as paragraph to section 5 to set the scene: we use enoder-decoder NMT....}
In this Section we introduce the basics of NMT, as well as some necessary terminology and notation that will be used throughout the paper.
Most work on NMT is based on the sequence-to-sequence approach with encoder and decoder networks \cite{sutskever2014sequence}. The encoder maps the input sequence $\vec{x}$ consisting of $I$ words ${x_1,...,x_I}$ into a sequence of hidden states $z={z_1,...,z_I}$, which is summarized into a single vector using attention mechanism \cite{bahdanau2014neural,vaswani2017attention}. Given $\vec{z}$ the decoder generates an output sequence $\vec{y}={y_1,...,y_T}$. The probability of generating $\vec{y}$ is factorized as follows:
\begin{equation}
p(\vec{y}|\vec{x},\theta) = \prod_{t=1}^{T} p(y_t|\vec{y}_{<t},\vec{x},\theta)
\end{equation}
where $\theta$ represents model parameters. The decoder produces the probability distribution $p(y_t|\vec{y}_{<t},\vec{x},\theta)$ over system vocabulary at each time step using \emph{softmax function}. The model is trained to minimize cross-entropy loss:
\begin{equation}
\mathcal{L}=-\sum_{t=1}^T \log p(y_t|\vec{y}_{<t},\vec{x},\theta)
\end{equation}

Several neural network architectures have been proposed for NMT over the recent years \cite{bahdanau2014neural,luong2015effective,gehring2017convolutional,vaswani2017attention}. Throughout Sections \ref{sec:unsupervised_quality_estimation} and \ref{sec:experiments} we present unsupervised quality indicators that can be extracted from any attention-based encoder-decoder NMT model, whereas Section 
\ref{subsec:results_uncertainty_models}
looks at some of the existing NMT system variants to study whether model architecture and training affects the correlation of output probabilities with perceived translation quality.


==> tables/attention_table_all_languages_split3.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c}
                & et-en & ro-en & si-en & ne-en & en-de & en-zh \\ \hline
AW:Ent-Max      &  0.323 &\textbf{0.526}  & 0.081  & 0.265  & -0.056* & 0.067 \\
AW:Ent-Avg      &  0.371 &0.383  & 0.097  & 0.205  & -0.054* & 0.112\\
best head/layer &  \textbf{0.411} &\textbf{0.638}  & \textbf{0.255}  & \textbf{0.381}  & 0.013*  & \textbf{0.168} 
\end{tabular}%
}
\caption{Pearson correlation coefficient; zscore, 1K, split3. Bold marks measurements that significantly outperform others. (*) marks values with high p-value(>0.05)}
\label{tab:PCC_zscore_1K_alllang_split3}
\end{table*}

==> tables/attention_tables_across_langs_10K.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c}
 & et-en & ro-en & si-en & ne-en & en-de & en-zh \\ \hline
AW:AvgAW-Ent & 0.247 & 0.249 & 0.106 & 0.186 & 0.057 & 0.149 \\
AW:MaxAW-Ent & 0.223 & 0.281 & 0.129 & 0.102 & 0.062 & 0.139 \\
AW:Ent-Max & 0.284 & \textbf{0.486} & 0.092 & 0.228 & 0.018* & 0.112 \\
AW:Ent-Avg & 0.299 & 0.347 & 0.099 & 0.192 & 0.05 & 0.184 \\
best head/layer & \textbf{0.345} & 0.552 & \textbf{0.250} & \textbf{0.298} & 0.076 & \textbf{0.217}
\end{tabular}%
}
\caption{Pearson correlation coefficient; zscore, 10K. Bold marks measurements that significantly outperform others. (*) marks values with high p-value(>0.05)}
\label{tab:PCC_zscore_10K_alllang}
\end{table*}

==> tables/attention_tables_eten_10K.tex <==
\begin{table*}[h!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\multirow{2}{*}{}                & \multicolumn{2}{c|}{H1}                                                                                & \multicolumn{2}{c|}{H2}                                                                                & \multicolumn{2}{c|}{H3}                                                                                & \multicolumn{2}{c|}{H4}                                                                                & \multicolumn{2}{c|}{H5}                                                                                & \multicolumn{2}{c|}{H6}                                                                                & \multicolumn{2}{c|}{H7}                                                                                & \multicolumn{2}{c|}{H8}                                                                                & \multicolumn{2}{c|}{avg over heads}                                                                    & \multicolumn{2}{c}{max over heads}                                                                       \\ \cline{2-21} 
                                 & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} \\ \hline

Layer 1 & 0.205 & 0.223 & 0.148 & 0.157 & 0.163 & 0.168 & 0.202 & 0.205 & 0.226 & 0.229 & 0.157 & 0.174 & 0.218 & 0.226 & 0.244 & 0.247 & 0.195 & 0.206 & 0.202 & 0.210  \\


Layer 2 & 0.228 & 0.232 & \textbf{0.337} & \textbf{0.336} & 0.196 & 0.216 & 0.134 & 0.149 & 0.188 & 0.192 & 0.162 & 0.167 & 0.196 & 0.199 & 0.217 & 0.222 & 0.195 & 0.210 & 0.221 & 0.227  \\


Layer 3 & 0.217 & 0.230 & 0.253 & 0.274 & 0.233 & 0.237 & 0.249 & 0.246 & 0.238 & 0.237 & 0.243 & 0.251 & 0.293 & 0.315 & 0.257 & 0.265 & 0.257 & 0.271 & 0.256 & 0.264  \\


Layer 4 & 0.127 & 0.131 & 0.285 & 0.296 & 0.273 & 0.282 & 0.215 & 0.225 & 0.241 & 0.244 & 0.235 & 0.256 & 0.223 & 0.230 & 0.214 & 0.219 & 0.287 & 0.292 & 0.286 & 0.288  \\


Layer 5 & 0.154 & 0.172 & 0.135 & 0.187 & 0.281 & 0.264 & 0.249 & 0.280 & 0.259 & 0.276 & 0.180 & 0.204 & 0.196 & 0.168 & 0.211 & 0.225 & 0.251 & 0.260 & 0.272 & 0.272  \\


Layer 6 & 0.137 & 0.174 & 0.147 & 0.208 & 0.159 & 0.173 & 0.178 & 0.190 & 0.160 & 0.177 & 0.225 & 0.233 & 0.134 & 0.191 & 0.169 & 0.165 & 0.191 & 0.200 & 0.236 & 0.232  \\


avg over layers & 0.229 & 0.237 & 0.251 & 0.253 & 0.231 & 0.244 & 0.243 & 0.249 & 0.247 & 0.250 & 0.239 & 0.249 & 0.234 & 0.238 & 0.254 & 0.261 & 0.234 & 0.242 & 0.223 & 0.230  \\


max over layers & 0.232 & 0.237 & 0.244 & 0.246 & 0.235 & 0.244 & 0.236 & 0.242 & 0.246 & 0.249 & 0.239 & 0.241 & 0.239 & 0.242 & 0.261 & 0.268 & 0.232 & 0.238 & 0.215 & 0.217  \\


\end{tabular}%
}
\caption{Pearson correlation coefficients between \texttt{Att-Ent} (computed from Encoder-Decoder attention weights) and DA scores for Estonian-English Transformer model. For cells that combine average over heads and maximum over layers or vice versa, we first compute the corresponding value for heads and then for layers.}
\label{tab:AW-Ent-PCC-eten}
\end{table*}



\begin{table*}[h!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\multirow{2}{*}{}                & \multicolumn{2}{c|}{H1}                                                                                & \multicolumn{2}{c|}{H2}                                                                                & \multicolumn{2}{c|}{H3}                                                                                & \multicolumn{2}{c|}{H4}                                                                                & \multicolumn{2}{c|}{H5}                                                                                & \multicolumn{2}{c|}{H6}                                                                                & \multicolumn{2}{c|}{H7}                                                                                & \multicolumn{2}{c|}{H8}                                                                                & \multicolumn{2}{c|}{avr over heads}                                                                    & \multicolumn{2}{c}{max over heads}                                                                       \\ \cline{2-21} 
                                 & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} \\ \hline

Layer 1 & 0.230 & 0.246 & 0.173 & 0.181 & 0.196 & 0.200 & 0.228 & 0.231 & 0.246 & 0.249 & 0.181 & 0.196 & 0.242 & 0.249 & 0.267 & 0.270 & 0.221 & 0.231 & 0.229 & 0.235  \\


Layer 2 & 0.252 & 0.256 & \textbf{0.346} & \textbf{0.346} & 0.219 & 0.237 & 0.162 & 0.173 & 0.215 & 0.219 & 0.180 & 0.181 & 0.216 & 0.220 & 0.238 & 0.243 & 0.219 & 0.233 & 0.244 & 0.250  \\


Layer 3 & 0.241 & 0.253 & 0.264 & 0.283 & 0.256 & 0.260 & 0.262 & 0.257 & 0.260 & 0.258 & 0.271 & 0.278 & 0.292 & 0.316 & 0.276 & 0.283 & 0.281 & 0.293 & 0.278 & 0.286  \\


Layer 4 & 0.126 & 0.128 & 0.299 & 0.307 & 0.289 & 0.298 & 0.225 & 0.235 & 0.248 & 0.250 & 0.227 & 0.252 & 0.232 & 0.237 & 0.222 & 0.225 & 0.302 & 0.305 & 0.302 & 0.304  \\


Layer 5 & 0.144 & 0.164 & 0.131 & 0.187 & 0.291 & 0.274 & 0.249 & 0.284 & 0.264 & 0.279 & 0.182 & 0.207 & 0.207 & 0.179 & 0.211 & 0.226 & 0.259 & 0.267 & 0.283 & 0.282  \\


Layer 6 & 0.140 & 0.181 & 0.149 & 0.221 & 0.170 & 0.188 & 0.180 & 0.192 & 0.160 & 0.177 & 0.232 & 0.238 & 0.127 & 0.191 & 0.175 & 0.171 & 0.201 & 0.208 & 0.247 & 0.241  \\


avg over layers & 0.248 & 0.254 & 0.270 & 0.270 & 0.255 & 0.267 & 0.265 & 0.269 & 0.267 & 0.270 & 0.261 & 0.269 & 0.252 & 0.253 & 0.272 & 0.276 & 0.255 & 0.261 & 0.246 & 0.252  \\


max over layers & 0.254 & 0.259 & 0.263 & 0.264 & 0.259 & 0.266 & 0.260 & 0.263 & 0.267 & 0.270 & 0.261 & 0.262 & 0.258 & 0.259 & 0.281 & 0.287 & 0.255 & 0.259 & 0.239 & 0.241  \\


\end{tabular}%
}
\caption{Spearman correlation coefficients between \texttt{Att-Ent} (computed from Encoder-Decoder attention weights) and DA scores for Estonian-English Transformer model. For cells that combine average over heads and maximum over layers or vice versa, we first compute the corresponding value for heads and then for layers.} %To get average/maxpooling over heads and over layers, we first compute average/maxpooling over heads and then over layers.}
\label{tab:AW-Ent-SCC-eten}
\end{table*}

==> tables/attention_tables_roen_10K.tex <==
\begin{table*}[h!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\multirow{2}{*}{}                & \multicolumn{2}{c|}{H1}                                                                                & \multicolumn{2}{c|}{H2}                                                                                & \multicolumn{2}{c|}{H3}                                                                                & \multicolumn{2}{c|}{H4}                                                                                & \multicolumn{2}{c|}{H5}                                                                                & \multicolumn{2}{c|}{H6}                                                                                & \multicolumn{2}{c|}{H7}                                                                                & \multicolumn{2}{c|}{H8}                                                                                & \multicolumn{2}{c|}{avg over heads}                                                                    & \multicolumn{2}{c}{max over heads}                                                                       \\ \cline{2-21} 
                                 & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} \\ \hline

Layer 1 & 0.229 & 0.086 & 0.245 & 0.122 & 0.192 & 0.081 & 0.188 & 0.180 & 0.126 & 0.149 & 0.160 & 0.175 & 0.271 & 0.245 & 0.484 & 0.520 & 0.209 & 0.243 & 0.288 & 0.356  \\


Layer 2 & 0.087 & 0.023 & -0.001 & 0.199 & 0.109 & 0.023 & 0.153 & 0.116 & 0.074 & 0.200 & -0.063 & 0.122 & 0.450 & \textbf{0.544} & 0.167 & 0.316 & -0.020 & 0.165 & 0.151 & 0.290  \\


Layer 3 & -0.200 & -0.107 & -0.007 & 0.285 & 0.191 & 0.427 & -0.255 & 0.194 & -0.091 & 0.184 & 0.378 & 0.474 & 0.120 & 0.076 & -0.018 & 0.364 & -0.141 & 0.248 & -0.021 & 0.210  \\


Layer 4 & -0.067 & 0.188 & 0.186 & 0.396 & -0.095 & 0.424 & 0.192 & 0.392 & -0.031 & 0.237 & -0.012 & 0.104 & -0.012 & 0.343 & -0.211 & 0.030 & -0.174 & 0.234 & -0.107 & 0.255  \\


Layer 5 & 0.185 & 0.378 & 0.030 & 0.270 & 0.239 & 0.435 & 0.134 & 0.198 & 0.142 & 0.221 & 0.067 & 0.448 & 0.269 & 0.381 & 0.098 & 0.368 & 0.039 & 0.365 & 0.131 & 0.347  \\


Layer 6 & 0.213 & 0.184 & 0.246 & 0.167 & 0.330 & 0.251 & 0.032 & 0.170 & 0.311 & 0.423 & 0.116 & 0.103 & 0.288 & 0.247 & 0.320 & 0.216 & 0.164 & 0.229 & 0.181 & 0.253  \\


avg over layers & -0.045 & 0.078 & -0.012 & 0.287 & -0.059 & 0.322 & -0.034 & 0.208 & 0.012 & 0.235 & -0.068 & 0.270 & 0.065 & 0.430 & -0.060 & 0.291 & -0.058 & 0.247 & 0.037 & 0.287  \\


max over layers & 0.023 & 0.137 & 0.124 & 0.317 & 0.133 & 0.345 & 0.090 & 0.267 & 0.158 & 0.301 & 0.173 & 0.356 & 0.223 & 0.445 & 0.107 & 0.338 & 0.118 & 0.316 & 0.199 & 0.279  \\


\end{tabular}%
}
\caption{Pearson correlation coefficients between \texttt{Att-Ent} (computed from Encoder-Decoder attention weights) and DA scores for Romanian-English Transformer model. For cells that combine average over heads and maximum over layers or vice versa, we first compute the corresponding value for heads and then for layers. Number of sentences: 10000}
\label{tab:AW-Ent-PCC-roen-10K}
\end{table*}


\begin{table*}[h!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc}
\multirow{2}{*}{}                & \multicolumn{2}{c|}{H1}                                                                                & \multicolumn{2}{c|}{H2}                                                                                & \multicolumn{2}{c|}{H3}                                                                                & \multicolumn{2}{c|}{H4}                                                                                & \multicolumn{2}{c|}{H5}                                                                                & \multicolumn{2}{c|}{H6}                                                                                & \multicolumn{2}{c|}{H7}                                                                                & \multicolumn{2}{c|}{H8}                                                                                & \multicolumn{2}{c|}{avg over heads}                                                                    & \multicolumn{2}{c}{max over heads}                                                                       \\ \cline{2-21} 
                                 & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}with\\ EOS\end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o\\ EOS\end{tabular} \\ \hline

Layer 1 & 0.216 & 0.128 & 0.235 & 0.151 & 0.148 & 0.125 & 0.153 & 0.197 & 0.072 & 0.175 & 0.176 & 0.182 & 0.250 & 0.252 & 0.412 & 0.408 & 0.194 & 0.246 & 0.261 & 0.320 \\


Layer 2 & 0.116 & 0.083 & 0.079 & 0.227 & 0.127 & 0.101 & 0.085 & 0.153 & 0.124 & 0.210 & 0.031 & 0.164 & 0.355 & \textbf{0.392} & 0.205 & 0.281 & 0.067 & 0.190 & 0.175 & 0.270  \\


Layer 3 & -0.102 & 0.050 & 0.090 & 0.300 & 0.206 & 0.331 & 0.056 & 0.227 & -0.003 & 0.215 & 0.291 & 0.321 & 0.195 & 0.136 & 0.171 & 0.328 & 0.071 & 0.257 & 0.096 & 0.215  \\


Layer 4 & 0.068 & 0.169 & 0.106 & 0.221 & 0.016 & 0.324 & 0.209 & 0.324 & 0.104 & 0.223 & 0.051 & 0.195 & 0.075 & 0.208 & -0.055 & 0.134 & 0.037 & 0.212 & 0.062 & 0.215  \\


Layer 5 & 0.200 & 0.300 & 0.060 & 0.216 & 0.192 & 0.343 & 0.146 & 0.238 & 0.197 & 0.179 & 0.102 & 0.339 & 0.225 & 0.282 & 0.185 & 0.301 & 0.133 & 0.298 & 0.193 & 0.291 \\


Layer 6 & 0.224 & 0.172 & 0.252 & 0.210 & 0.309 & 0.207 & 0.087 & 0.190 & 0.246 & 0.333 & 0.139 & 0.138 & 0.242 & 0.213 & 0.267 & 0.175 & 0.199 & 0.213 & 0.202 & 0.236 \\


avg over layers & 0.065 & 0.118 & 0.096 & 0.278 & 0.060 & 0.290 & 0.040 & 0.220 & 0.099 & 0.216 & 0.065 & 0.259 & 0.207 & 0.360 & 0.135 & 0.280 & 0.076 & 0.240 & 0.116 & 0.266 \\


max over layers & 0.094 & 0.159 & 0.172 & 0.293 & 0.169 & 0.300 & 0.130 & 0.257 & 0.176 & 0.265 & 0.201 & 0.308 & 0.263 & 0.372 & 0.205 & 0.312 & 0.166 & 0.287 & 0.211 & 0.263 \\


\end{tabular}%
}
\caption{Spearman correlation coefficients between \texttt{Att-Ent} (computed from Encoder-Decoder attention weights) and DA scores for Romanian-English Transformer model. For cells that combine average over heads and maximum over layers or vice versa, we first compute the corresponding value for heads and then for layers. Number of sentences: 10000}
\label{tab:AW-Ent-SCC-roen-10K}
\end{table*}

==> tables/nmt_models_da_separate.tex <==
\begin{table}[h]
\small
\begin{center}
\begin{tabular}{||l | c c ||} 
\hline
& $r$ & $r_s$ \\ 
\hline\hline
Transformer & 0.482 & 0.481\\
RNN & 0.502 & 0.508\\
Transformer-ensemble & 0.538 & 0.528\\
Transformer-MoE & 0.429 & 0.426\\
Transformer-MoE-all & 0.449 & 0.449\\
Transformer-sampling & 0.533 & 0.536\\
Transformer-dbeam & 0.424 & 0.457\\
Transformer-temperature & 0.536 & 0.534\\
Transformer-multilingual & 0.428 & 0.426\\ % absolute correlation
\hline
\end{tabular}
\end{center}
\caption{Pearson and Spearman correlation between softmax output probabilities and DA judgments for translations generated by different NMT models described in Section \ref{sec:models}}
\label{tab:uncertainty_across_models}
\end{table}

\begin{table}[h]
\begin{center}
\begin{tabular}{||l | r r ||} 
\hline
& \textbf{DA-abs} & \textbf{DA-z} \\ 
\hline\hline
Transformer & 58.88 & 0.122\\
RNN & 43.63 & -0.403\\
Transformer-ensemble & 61.19 & 0.197\\
Transformer-MoE & 51.20 & -0.148\\
Transformer-sampling & 42.02 & -0.465\\
Transformer-dbeam & 55.12 & -0.005\\
Transformer-temperature & 58.23 & 0.112\\
\hline
\end{tabular}
\end{center}
\caption{Average DA scores for the translations generated by the NMT systems described in Section \ref{sec:models}. DA-abs corresponds to absolute DA judgments produced on the scale 1-100 and DA-z corresponds to standardized DA scores.}
\label{tab:da_across_models}
\end{table}


==> tables/summary_table_all_languages.tex <==
\begin{table*}
\small
\begin{center}
\begin{tabular}{|l | c c c c c c|} 
\hline
& eten & roen & sien & neen & ende & enzh\\ 
\hline
$\mathrm{TP}$ & 0.435 & 0.545 & 0.399 & 0.385 & 0.149 & 0.291 \\
$\mathrm{Soft\mbox{-}Ent}$ & -0.352 & -0.494 & -0.441 & -0.399 & -0.126 & -0.359 \\ % This is much lower than before: double-check!
$\mathrm{Sent\mbox{-}Var}$ & -0.458 & -0.550 & -0.410 & -0.356 & -0.140 & -0.351 \\
\hline
$\mathrm{D\mbox{-}TP}$ & 0.558 & 0.622 & 0.439 & 0.418 & 0.177 & 0.325 \\
$\mathrm{D\mbox{-}Var}$ & -0.451 & -0.465 & -0.361 & -0.290 & -0.115 & -0.276 \\
% $\mathrm{D\mbox{-}Combo}$ & 0.516 & 0.611 & 0.441 & 0.418 & 0.180 & 0.331 \\
$\mathrm{D\mbox{-}Combo\mbox{-}Wang}$ & -0.462 & -0.479 & -0.362 & -0.291 & -0.117 & -0.280 \\
$\mathrm{D\mbox{-}Ling\mbox{-}Sim}$ & 0.544 & 0.657 & 0.361 & 0.352 & 0.141 & 0.337 \\ % differences with D-TP are not significant
\hline
$\mathrm{AW\mbox{:}AvgAW\mbox{-}Ent}$        & 0.250         & 0.256 & 0.127 &0.125 &0.074 &  0.184\\
$\mathrm{AW\mbox{:}MaxAW\mbox{-}Ent}$        & 0.236         & 0.267 & 0.145 &0.050 &0.066 &  0.184\\
%$\mathrm{AW\mbox{:}MaxAW\mbox{-}Max}$        & 0.205         & 0.314 & 0.045 &0.209 & 0 & 0\\
%$\mathrm{AW\mbox{:}MaxAW\mbox{-}Avg}$        & 0.278         & 0.357 & 0.048 &0.13  & 0 & 0.125\\
$\mathrm{AW\mbox{:}Ent\mbox{-}Max}$          & 0.256         & 0.388 & 0.06  &0.221 &0     & 0.099\\
$\mathrm{AW\mbox{:}Ent\mbox{-}Avg}$          & \textbf{0.297}& 0.350 & 0.105 &0.111 &0.08  & 0.217\\
$\mathrm{AW\mbox{:}\text{best head/layer}}$  & \textbf{0.339}& 0.455 & 0.228 &0.286 &0.088 & 0.259\\
\hline
% $\mathrm{LASER}$ &  &  \\
$\mathrm{OpenKiwi}$ & 0.454 & 0.557 & 0.371 & 0.328 & & \\
\hline
$\mathrm{sentBLEU}$ & 0.361 & & & & &\\
$\mathrm{ChrF}$ & 0.440 & & & & &\\
$\mathrm{Meteor}$ & 0.444 & & & & &\\
\hline
\end{tabular}
\end{center}
\caption{Spearman ($r_s$) correlation between unsupervised QE indicators and human DA judgments. MC dropout measures are computed with 30 inference passes.}
\label{tab:uncertainty_indicators}
\end{table*}


==> tables/summary_table_all_languages_pearson.tex <==
\begin{table*}[t]
\begin{center}
% \small
\footnotesize
\begin{tabular}{l l | c c c c c c} 
%\hline
& & \multicolumn{2}{c}{Mid-resource} & \multicolumn{2}{c}{Low-resource} & \multicolumn{2}{c}{High-resource}\\
& & Et-En & Ro-En & Si-En & Ne-En & En-De & En-Zh\\ 
\hline \hline
\multicolumn{8}{c}{Unsupervised QE} \\
\hline
& $\mathrm{TP}$ & \textbf{0.424} & \textbf{0.616} & 0.399 & 0.367 & 0.117 & 0.276 \\  % 0.145 
I & $\mathrm{Soft\mbox{-}Ent}$ (-) & 0.357 & 0.582 & \underline{\textbf{0.447}} & \textbf{0.404} & \underline{\textbf{0.162}} & \underline{\textbf{0.347}} \\  % 0.118
& $\mathrm{Sent\mbox{-}Var}$ (-) & 0.416 & 0.577 & \textbf{0.423} & \textbf{0.376} & 0.074 & 0.321 \\  %\underline{\textbf{0.173}}
\hline
& $\mathrm{D\mbox{-}TP}$ & \underline{\textbf{0.520}} & \underline{\textbf{0.649}} & \textbf{0.442} & \underline{\textbf{0.416}} & \textbf{0.126} & \textbf{0.313} \\ % \textbf{0.166}
II & $\mathrm{D\mbox{-}Var}$ (-) & 0.259 & 0.465 & 0.284 & 0.154 & 0.033 & 0.161\\ % 0.043
& $\mathrm{D\mbox{-}Combo}$ (-) & 0.421 & 0.382 & 0.304 & 0.337 & 0.047 & 0.135 \\ % 0.122
& $\mathrm{D\mbox{-}Lex\mbox{-}Sim}$ & \underline{\textbf{0.508}} & \underline{\textbf{0.664}} & 0.363 & 0.375 & \textbf{0.122} & 0.285 \\ % for en-de results for wmt21 are reported
\hline
% & $\mathrm{AW\mbox{:}AvgAW\mbox{-}Ent}$       &0.240  &0.240  &0.118  &0.160 &0.056 &0.146\\
% & $\mathrm{AW\mbox{:}MaxAW\mbox{-}Ent}$       &0.218  &0.270  &0.142  &0.094 &0.061 &0.151\\
%$\mathrm{AW\mbox{:}MaxAW\mbox{-}Max}$       &0.221  &0.514  &0.07   &0.21  &0     &0\\
%%$\mathrm{AW\mbox{:}MaxAW\mbox{-}Avg}$       &0.289  &0.505  &0.05   &0.144 &0     &0.089\\
III & $\mathrm{AW\mbox{:}Ent\mbox{-}Max}$         &0.271  &\textbf{0.497}  &0.08   &0.225 &0.001 &0.07\\
& $\mathrm{AW\mbox{:}Ent\mbox{-}Avg}$         &0.299  &0.354  &0.107  &0.138 &0.048 &\textbf{0.178}\\
& $\mathrm{AW\mbox{:}\text{best head/layer}}$ &\textbf{0.354} &\textbf{0.568}  &\textbf{0.263}  &\textbf{0.309} &0.086 &\textbf{0.219}\\
\hline\hline
\multicolumn{8}{c}{Supervised QE} \\
\hline
& $\mathrm{OpenKiwi}$ & 0.475 & \underline{0.628} & 0.369 & \underline{0.370} & 0.009 & 0.313\\ \hline\hline
\multicolumn{8}{c}{Reference-based metrics} \\
& $\mathrm{sentBLEU}$ & 0.357 & - & - & - & - & -\\
& $\mathrm{TER}$ (-) & 0.380 & - & - & - & - & - \\
& $\mathrm{ChrF}$ & \textbf{0.444} & - & - & - & - & -\\
& $\mathrm{Meteor}$ & \textbf{0.470} & - & - & - & - & -\\
\end{tabular}
\end{center}
\caption{Pearson ($r$) correlation between unsupervised QE indicators and human DA judgments. Results not significantly outperformed by any other measure are underlined; results not significantly outperformed by any other measure from the same group are marked in bold.}% Significance is computed with Hotelling-Williams test \cite{Williams:1959}.}
\label{tab:uncertainty_indicators}
\end{table*}

% \todo{Table 1: remove AW from attention metrics? too long.}


==> tables/summary_table_all_languages_pearson_remove_metrics.tex <==
\renewcommand{\arraystretch}{1.1}
\begin{table*}[t]
\begin{center}
\small
% \footnotesize
\begin{tabular}{l l | c c c c c c} 
%\hline
& & \multicolumn{2}{c}{Mid-resource} & \multicolumn{2}{c}{Low-resource} & \multicolumn{2}{c}{High-resource}\\
& & Et-En & Ro-En & Si-En & Ne-En & En-De & En-Zh\\ 
\hline \hline
% \multicolumn{8}{c}{Unsupervised QE} \\
% \hline
& $\mathrm{TP}$ & \textbf{0.424} & \textbf{0.616} & 0.399 & 0.367 & 0.117 & 0.276 \\  % 0.145 
I & $\mathrm{Soft\mbox{-}Ent}$ (-) & 0.357 & 0.582 & \underline{\textbf{0.447}} & \textbf{0.404} & \underline{\textbf{0.162}} & \underline{\textbf{0.347}} \\  % 0.118
& $\mathrm{Sent\mbox{-}Var}$ (-) & 0.416 & 0.577 & \textbf{0.423} & \textbf{0.376} & 0.074 & 0.321 \\  %\underline{\textbf{0.173}}
\hline
& $\mathrm{D\mbox{-}TP}$ & \underline{\textbf{0.520}} & \underline{\textbf{0.649}} & \textbf{0.442} & \underline{\textbf{0.416}} & \textbf{0.126} & \textbf{0.313} \\ % \textbf{0.166}
II & $\mathrm{D\mbox{-}Var}$ (-) & 0.259 & 0.465 & 0.284 & 0.154 & 0.033 & 0.161\\ % 0.043
& $\mathrm{D\mbox{-}Combo}$ (-) & 0.421 & 0.382 & 0.304 & 0.337 & 0.047 & 0.135 \\ % 0.122
& $\mathrm{D\mbox{-}Lex\mbox{-}Sim}$ & \underline{\textbf{0.508}} & \underline{\textbf{0.664}} & 0.363 & 0.375 & \textbf{0.122} & 0.285 \\ % differences with D-TP are not significant  %\textbf{0.140}
\hline
III & $\mathrm{AW\mbox{:}Ent\mbox{-}Max}$         &0.271  &\textbf{0.497}  &0.08   &0.225 &0.001 &0.070\\
& $\mathrm{AW\mbox{:}Ent\mbox{-}Avg}$         &0.299  &0.354  &0.107  &0.138 &0.048 &\textbf{0.178}\\
& $\mathrm{AW\mbox{:}\text{best head/layer}}$ &\textbf{0.354} &\textbf{0.568}  &\textbf{0.263}  &\textbf{0.309} &0.086 &\textbf{0.219}\\
\hline\hline
% \multicolumn{8}{c}{Supervised QE} \\
% \hline
& $\mathrm{OpenKiwi}$ & 0.475 & \underline{0.628} & 0.369 & \underline{0.370} & 0.009 & 0.313\\ \hline\hline
\end{tabular}
\end{center}
% \caption{Pearson ($r$) correlation between unsupervised QE indicators and human DA judgments. MC dropout measures are computed with 30 inference passes. Bold marks measurements not significantly outperformed by any other from the same group; measurements not significantly outperformed by any other overall, are underlined. Significance is computed with Hotelling-Williams test \cite{Williams:1959}.}
% \caption{Pearson ($r$) correlation between unsupervised QE indicators and human DA judgments.} 
\caption{Pearson ($r$) correlation between unsupervised QE indicators and human DA judgments. Bold marks measurements not significantly outperformed by any other from the same group; measurements not significantly outperformed by any other overall, are underlined.} 
\label{tab:uncertainty_indicators}
\end{table*}

% \todo{Table 1: remove AW from attention metrics? too long.}


==> tables/summary_table_eten.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{|l | c c |} 
\hline
& $r$ & $r_s$ \\ 
\hline
$\mathrm{TP}$ & \textbf{0.409} & \textbf{0.415} \\  % These are the results for the 10K segments
$\mathrm{Soft\mbox{-}Ent}$ & \textcolor{red}{-0.359} & -0.359\\ % This is much lower than before: double-check!
$\mathrm{Sent\mbox{-}Var}$ & -0.394 & -0.422\\
\hline
$\mathrm{D\mbox{-}TP}$ & \textbf{0.493} & \textbf{0.515}\\
$\mathrm{D\mbox{-}Var}$ & \textcolor{red}{-0.255} & -0.407 \\
$\mathrm{D\mbox{-}Combo}$ & \textbf{0.489} & \textbf{0.516}\\
$\mathrm{D\mbox{-}Combo\mbox{-}Wang}$ & -0.363 & -0.416\\
$\mathrm{D\mbox{-}Ling\mbox{-}Sim}$ & 0.460 & 0.501 \\
\hline
$\mathrm{AW\mbox{:}AvgAW\mbox{-}Ent}$ & 0.242 & 0.261 \\
$\mathrm{AW\mbox{:}MaxAW\mbox{-}Ent}$ & 0.217 & 0.241 \\
$\mathrm{AW\mbox{:}MaxAW\mbox{-}Max}$ & 0.218 & 0.211 \\
$\mathrm{AW\mbox{:}MaxAW\mbox{-}Avg}$ & 0.270 & 0.277 \\
$\mathrm{AW\mbox{:}Ent\mbox{-}Max}$ & 0.278 & 0.279 \\
$\mathrm{AW\mbox{:}Ent\mbox{-}Avg}$ & \textbf{0.291} & \textbf{0.306} \\
$\mathrm{AW\mbox{:}\text{best head/layer}}$ & \textbf{0.336} & \textbf{0.346} \\
\hline
% $\mathrm{LASER}$ &  &  \\
$\mathrm{OpenKiwi}$ & 0.472 & 0.454 \\
$\mathrm{DeepQuest}$ & &  \\
\hline
$\mathrm{sentBLEU}$ & 0.359 & 0.367 \\
$\mathrm{ChrF}$ & 0.444 & 0.438 \\
$\mathrm{Meteor}$ & \textcolor{red}{0.392} & 0.505 \\
\hline
\end{tabular}
\end{center}
\caption{Pearson ($r$) and Spearman ($r_s$) correlation between unsupervised QE indicators and human DA judgments for Estonian-English Transformer model. MC dropout measures are computed with 30 inference passes.}
\label{tab:uncertainty_indicators}
\end{table}


==> uncertainty.tex <==
% \subsection{Uncertainty}
\subsection{Quantifying Uncertainty}
\label{subsec:uncertainty}

% Above we assumed the NMT probabilities are well calibrated and therefore can be a good indicator of MT output quality. This might not be the case, as recent studies suggest that modern neural networks may be poorly calibrated \cite{nguyen2015posterior,guo2017calibration,lakshminarayanan2017simple}. Superior results for unsupervised QE can be achieved by improving uncertainty quantification. We explore a widely used approach to approximate Bayesian inference proposed by \citet{gal2016dropout}. We also look at a simple non-Bayesian method for calibrating predictive probabilities called temperature scaling \cite{platt1999probabilistic,guo2017calibration}. 

It has been argued in recent work that deep neural networks do not properly represent model uncertainty \cite{gal2016dropout,lakshminarayanan2017simple}. Uncertainty quantification in deep learning typically relies on Bayesian formalism \cite{mackay1992bayesian,graves2011practical,welling2011bayesian,gal2016dropout,tran2019bayesian}. Bayesian NNs learn a posterior distribution over parameters that quantifies \emph{model} or \emph{epistemic} uncertainty, i.e. our lack of knowledge as to which model generated the training data.\footnote{A distinction is typically made between epistemic and aleatoric uncertainty, where the latter captures the noise inherent to the observation \cite{kendall2017uncertainties}. We leave modelling aleatoric uncertainty in NMT for future work.} To avoid changing the NMT training procedure, %instead of using Bayesian networks we explore an approximation to Bayesian inference called Monte Carlo dropout.
instead of using Bayesian networks which usually come with prohibitive computational costs we explore an approximation to Bayesian inference called Monte Carlo (MC) dropout \cite{gal2016dropout}.

\paragraph{Monte Carlo Dropout}

% A standard way for reasoning about uncertainty in machine learning is to use Bayesian methods.

% Bayesian neural networks usually come with prohibitive computational costs and various approximations have been developed to alleviate this issue. One such approach developed by \citet{gal2016dropout} is called Monte Carlo (MC) dropout.
Dropout is a method introduced by \citet{srivastava2014dropout} to reduce overfitting when training deep NNs. It consists in randomly masking neurons to zero based on Bernoulli distribution. \citet{gal2016dropout} use dropout at test time before every weight layer. They perform several forward passes through the network and collect posterior probabilities generated by the model with parameters perturbed by dropout. Mean and variance of the resulting distribution can then be used to represent model uncertainty. %They show that this is mathematically equivalent to an approximation to the probabilistic deep Gaussian process.

We propose two flavours of MC dropout-based measures for unsupervised QE. \textbf{First}, we compute the expectation and variance for the set of probability estimates obtained by running $N$ stochastic forward passes through the MT model with model parameters $\hat{\theta}$ perturbed by dropout:%\paco{we need the correct $_n$ index}
\begin{equation}
\mathrm{D\mbox{-}TP} = \frac{1}{|N|} \sum_{n=1}^{N} \log p(\vec{y}^{(n)}|\vec{x},\hat{\theta})
\nonumber
\end{equation}
\begin{equation}
\mathrm{D\mbox{-}Var} = \frac{1}{|N|} \sum_{n=1}^{N} \log p(\vec{y}^{(n)}|\vec{x},\hat{\theta})^2 - \mathrm{D\mbox{-}TP}^2
\nonumber
\end{equation}

We also look at a combination of the two:
\begin{equation}
\mathrm{D\mbox{-}Combo} = \Big(1 - \frac{\mathrm{D\mbox{-}TP}}{\mathrm{D\mbox{-}Var}}\Big)
\nonumber
\end{equation}

% where $\hat{\theta}$ represents model parameters perturbed by dropout.

We note that these metrics have also been used by \citet{wang2019improving}, but with the purpose of minimising the effect of low quality outputs on NMT training with back translations.

\textbf{Second}, we measure lexical variation between the MT outputs generated for the same source segment when running inference with dropout. We posit that differences between likely MT hypotheses may also capture uncertainty and potential ambiguity and complexity of the source. We compute an average similarity ($sim$) score between the set $\{H\}$ of translation hypotheses as follows:

% \begin{equation}
% \mathrm{D\mbox{-}Ling\mbox{-}Sim} = C \sum_{h}^{H} \mathrm{METEOR}(h^i,h^j), i \neq j
% \end{equation}

\begin{equation}
\mathrm{D\mbox{-}Lex\mbox{-}Sim} = C\sum_{i=1}^{|H|} \sum_{j=1}^{|H|} sim(h_i,h_j)
\nonumber
\end{equation}

\noindent where $h_i, h_j \in H$, $i \ne j$ and $C=2^{-1}|H|(|H|-1)$ is the number of pairwise comparisons for $|H|$ hypotheses. We use Meteor \cite{denkowski2014meteor} to compute similarity scores.%, but any other similarity metric can be used for this purpose. 

\paragraph{Temperature Scaling}
% \paco{It's not clear to me why would temperature would improve calibration, maybe add a sentence to motivate better?}\mf{Added below}
Another popular approach to improving model calibration is temperature scaling, which consists in using a single corrective multiplicative factor for inputs to the softmax layer. Depending on the temperature value, this method can reduce the number of overconfident predictions by softening the softmax output. Formally:  % This is the same as in the models section!
\begin{equation}
\mathrm{TP\mbox{-}Temp} = \max\limits_{k} \sigma_{SM}(\vec{z}/Temp)^{(k)}
\nonumber
\end{equation}
where $\sigma_{SM}$ is the softmax function and $Temp$ is a scalar. With values $Temp > 1$ temperature scaling raises the output entropy, whereas values $Temp < 1$ result in "peakier" distributions. In our experiments we use $Temp=1.5$ that raises softmax output entropy resulting in higher uncertainty.\footnote{This value was obtained by computing correlation with Meteor automatic evaluation metric on a test partition of the training set for the MT systems, which is not used for our QE experiments.} Note that the value of $Temp$ does not change the maximum of the softmax function, and therefore, should not affect the predictions. However, due to the use of approximate search algorithms such as beam search in NMT, changing $Temp$ results in slightly different translations. For this reason, we discuss the results of temperature scaling in \S \ref{sec:discussion} as one of the system variants with a distinct set of human quality judgments. 

% a) keeping the original and the translation the same, we recalculate translation probabilities $N$ times for the same segment; b) keeping the original the same we generate $N$ translation outputs.

